Backdoors Stuck At The Frontdoor: Multi-Agent Backdoor Attacks That Backfire

Malicious agents in collaborative learning and outsourced data collection threaten the training of clean models. Backdoor attacks, where an attacker poisons a model during training to successfully achieve targeted misclassification, are a major concern to train-time robustness. In this paper, we investigate a multi-agent backdoor attack scenario, where multiple attackers attempt to backdoor a victim model simultaneously. A consistent backfiring phenomenon is observed across a wide range of games, where agents suffer from a low collective attack success rate. We examine different modes of backdoor attack configurations, non-cooperation / cooperation, joint distribution shifts, and game setups to return an equilibrium attack success rate at the lower bound. The results motivate the re-evaluation of backdoor defense research for practical environments.

==> 3.method_old.tex <==
\section{Multi-Agent Backdoor Attack}

\subsection{Game design}

% Game figure / diagram
% Pseudocode

In this section, we define the setup of the multi-agent backdoor attack in deep learning systems. 
In this multi-agent training regime, there two types of agents: defenders and participants. Participants can be classified as either attackers and non-attackers. To simplify the discussion and analysis, we evaluate the setup in terms of attackers and defenders (experimentally, a non-attacking participant would approximate a defender with larger dataset allocation). 
A multi-agent and single-agent attack are backdoor attacks with multiple and single attackers respectively.
The scope of our analysis is that the multi-agent backdoor attack is a single-turn game, composed of $N$ attackers and $M$ defenders. 
The game environment is a joint dataset $\mathbb{D}$ that agents contribute private datasets $D_i$ towards.
% ; the joint dataset and private dataset are denoted as $\mathbb{D}$-dataset and $D_i$-dataset respectively. 
After private dataset contributions are complete and $\mathbb{D}$ is set, the game ends and payoffs are computed with respect to test-time inputs evaluated on a model trained by the defender on $\mathbb{D}$.

\begin{figure}%[t!]
    \centering
    % \hspace{-1.5cm}
    \subfigure{\includegraphics[width=\linewidth]{assets/att_fig_2.pdf}}
    \caption{Representation of the multi-party backdoor attack. Attackers generate unique trigger patterns with target labels and contribute to a data pool for the defender to construct a model to be backdoor-triggered.}
    \label{fig:archi}
\end{figure}

\textbf{Attacker's Parameters: }
Each attacker is a player $\{a_{i}\}^{i \in N}$ that 
generates backdoored inputs $X^{\textnormal{poison}}$ to insert into their private dataset contribution $\{X^{\textnormal{poison}} \in D_i\}^{i \in N} \in \mathbb{D}$. 
Each attacker only has information with respect to their own private dataset source (including inputs, domain/style, class/labels), and backdoor trigger algorithm. 
Attackers use backdoor attack algorithm $b_i$, which accepts a set of inputs mapped to target poisoned labels $\{X_i:Y_i^{\textnormal{poison}}\} \in D_i$ to specify the intended label classification, backdoor perturbation rate $\varepsilon_i$ to specify the proportion of an input to be perturbed, and the poison rate $p_i$ to specify the proportion of the private dataset to contain backdoored inputs, to return $X^{\textnormal{poison}} = b_i(X_i, Y_i^{\textnormal{poison}}, \varepsilon_i, p_i)$. 
Details of $b_i$ are discussed in Appendix \ref{a1}.

An attacker $a_i$ would like to maximize their \textit{attack success rate} (ASR), which is the rate of misclassification of backdoored inputs $X^{\textnormal{poison}}$, from the clean label $Y_i^{\textnormal{clean}}$ to the target poisoned label $Y_i^{\textnormal{poison}}$, by the defender's model $f$.
The attacker prefers to keep poison rate $p_i$ low to generate imperceptible and stealthy perturbations.
% We can formalize the objective as $X_{backdoor} = \mathop{\arg\min}_{p} \{ b(X^{d_i}, Y^{d_i}, p) : f(X_{backdoor}) = Y^{d_i} \}$.
The attacker strategy, formulated by its actions, is denoted as $(\varepsilon_i, p_i, Y_i^{\textnormal{poison}}, b_i)$.
The predicted output would be $\widetilde{Y} = f(X_i; (\theta, \mathbb{D}); (r_j, s_j); (\varepsilon_i, p_i, Y_i^{\textnormal{poison}}, b_i))$. 
% In our experiments, we allocate datasets to each agent sampled from a single dataset (CIFAR10, unless otherwise specified), hence the choice of dataset is not specified as an action here; to simplify, if changes to the dataset are made, we assume here it is specified under $b_i$. 
We compute the accuracy of the predicted outputs in test-time against the target poisoned labels as the payoff $\pi = \max \texttt{Acc}(\widetilde{Y}, Y^{\textnormal{poison}})$.
% In a multi-agent setting, 
Each attacker optimizes their actions against the collective set of actions of the other $\neg i$ attackers.
% $N-1$ attackers, whose collective set of actions are denoted with the index $\neg i$. 
The payoff for each attacker $a_i$ is Eqt \ref{equation:attacker_obj}.
% in a multi-agent setting (Eqt \ref{equation:attacker_obj}) is thus:
% \begin{equation}
% \begin{split}
% \pi^{a_i} = 
% \max \texttt{Acc}(f(X_i; \mathbb{D}; (r_j, s_j); \{(\varepsilon_i, p_i, Y_i^{\textnormal{poison}}, b_i), \\ (\varepsilon_{\neg i}, p_{\neg i}, Y_{\neg i}^{\textnormal{poison}}, b_{\neg i}) \}), Y_i^{\textnormal{poison}})
% \end{split}
% \label{equation:attacker_obj}
% \end{equation}

\textbf{Defender's Parameters: }
Each defender is a player $\{d_{j}\}^{j \in M}$ that trains a model $f$ on the joint dataset $\mathbb{D}$, which may contain backdoored inputs, until it obtains model parameters $\theta$.
In our analysis, there is one defender only ($M=1$). 
In terms of information, the defender can view and access the joint dataset and contributions $\mathbb{D}$, % mention headers here only if agent-indexing
but is not given information on attacker actions (e.g. which inputs are poisoned).
% To formulate the defender's strategies $\{S_{j}(r)\}^{j \in M}$,
% the defender can sample from an action $r$, where an action is the choice of a defense method. 
To formulate the defender's strategies $\{(r_j, s_j)\}^{j \in M}$,
the defender can choose a model architecture (action $r_j$)
% (section \ref{3.2}), 
and backdoor defense (action $s_j$).
% and an action $s_j$ pertaining to the choice of a defense method (section \ref{3.5}). 
% These defenses are single-attacker backdoor defenses, and elaborated in section \ref{3.5}. 
The defender's primary objective is to minimize the individual and collective attack success rate of a set of attackers (maximize robustness accuracy against backdoored inputs), and its secondary objective to to retain and maximize standard accuracy against clean inputs.
Here, standard accuracy refers to the correct classification accuracy of the defender's model on clean inputs during run-time or inference-time. Robustness accuracy here refers to the accuracy of the model on backdoor-triggered inputs, i.e., high robustness accuracy means that the model can safely ignore triggers and predict the correct underlying label.
In this setup, we focus on minimizing the collective attack success rate, hence the defender's payoff can be approximated as the complementary of the mean attacker payoff (Eqt \ref{equation:defender_obj}).
% $\min \overline{\textnormal{Acc}}(f(\cdot), Y^{\textnormal{poison}})$
% $\pi^{d} = \min \frac{1}{N} \sum_i^{N} \texttt{Acc}(f(\cdot), Y_i^{\textnormal{poison}})$.
% \begin{equation}
% \begin{split}
% \pi^{d} = \min \frac{1}{N} \sum_i^{N} \texttt{Acc}(f(\cdot), Y_i^{\textnormal{poison}})
% \end{split}
% \label{equation:defender_obj}
% \end{equation}

\begin{numcases}{}
\begin{split}
\pi^{a_i} = 
\max \texttt{Acc}\Big(f(X_i; (\theta, \mathbb{D}); (r_j, s_j); \\ \{(\varepsilon_i, p_i, Y_i^{\textnormal{poison}}, b_i), \\ (\varepsilon_{\neg i}, p_{\neg i}, Y_{\neg i}^{\textnormal{poison}}, b_{\neg i}) \}), \\ Y_i^{\textnormal{poison}} \Big)  
\end{split}
\label{equation:attacker_obj}
\\
\begin{split}
\pi^{d} = \min \frac{1}{N} \sum_i^{N} \texttt{Acc}(f(\cdot), Y_i^{\textnormal{poison}})
\end{split}
\label{equation:defender_obj}
\end{numcases}

In experimental results, 
we denote the collective attacker payoff (a shorthand summary of the payoffs of individual attackers) and defender payoff
% In most figures (except those where we list out all the individual attacker payoffs), we represent the attacker payoff for each configuration 
as $\pi^{a} = \texttt{mean} \pm \texttt{std}$ and $\pi^{d} =((1-\texttt{mean}) \pm \texttt{std})$ respectively.
% , which is the collective attacker payoff, as well as a shorthand summary of the payoffs of individual attackers. 
% Defender payoffs can be evaluated as $\pi^{d} =((1-\texttt{mean}) \pm \texttt{std})$. 
In setups where attackers are only playing against attackers, the equilibrium $\widetilde{\pi}^{a_i, a_{\neg i}}$ is the collective payoff $\pi^{a}$ 
% where the collective ASR is 
of the highest value in the payoff matrix: $\widetilde{\pi}^{a_i, a_{\neg i}} = \texttt{max}(\texttt{mean} \pm \texttt{std})$.
For setups where attackers are playing against defenders, the equilibrium $\widetilde{\pi}^{a, d}$ is the collective payoff 
($\pi^{a}$, $\pi^{d}$)
% ($\texttt{mean} \pm \texttt{std}$, $(1-\texttt{mean}) \pm \texttt{std}$) 
where both payoff values are maximized with respect to the dominant strategy taken by the other. We demonstrate this procedure in Eqt \ref{equation:gta}, where we map strategy indices $q, u$ for each agent by $Q, U$ respectively:
$Q: q \mapsto (\varepsilon, p, Y^{\textnormal{poison}}, b)$, $U: u \mapsto (r, s)$.
% \begin{equation}
% \begin{split}
% \pi^{a, d} & = \{ \argmax_{i, j} \texttt{Acc}(a_i | d_j) \} \cap \{ \argmax_{i, j} \texttt{Acc}(d_j | a_i) \} \\
% & = \{ \argmax_{i, j} \texttt{Acc}(a_i | d_j) \} \cap \{ \argmin_{i, j} \texttt{Acc}(a_i | d_j) \}, \\ 
% & \phantom{========} {\small \textit{where } \texttt{Acc}(d_j | a_i) = 1 - \texttt{Acc}(a_i | d_j)}; \\
% & = \{ (i, j)_w \}^{w \in W} \cap \{ (i, j)_v \}^{v \in V} \\
% & = \{ (i, j)_{w=v} \}^{w, v \in W, V}
% \end{split}
% \label{equation:gta}
% \end{equation}
% 
\begin{equation}
\small
\begin{split}
\widetilde{\pi}^{a, d} & = \Big(\texttt{Acc}(Q(\widetilde{q}) | U(\widetilde{u})), \texttt{Acc}(U(\widetilde{u}) | Q(\widetilde{q}))\Big) \\
\widetilde{q}, \widetilde{u} & := \Big\{ \argmax_{q, u} \texttt{Acc}(Q(q) | U(u)) \Big\} \cap \Big\{ \argmax_{q, u} \texttt{Acc}(U(u) | Q(q)) \Big\} \\
& := \Big\{ \argmax_{q, u} \texttt{Acc}(Q(q) | U(u)) \Big\} \cap \Big\{ \argmin_{q, u} \texttt{Acc}(Q(q) | U(u)) \Big\}, \\ 
& \phantom{=========} {\textnormal{\textit{where} }  \texttt{Acc}(U(u) | Q(q)) = 1 - \texttt{Acc}(Q(q) | U(u))}; \\
& := \Big\{ (q, u)_w \Big\}^{w \in W} \cap \Big\{ (q, u)_v \Big\}^{v \in V} \\
& := \{ (q, u)_{w=v} \}^{w, v \in W, V}
\end{split}
\label{equation:gta}
\end{equation}
% 
\subsection{Distribution shift analysis}

% This paper (https://arxiv.org/pdf/2107.07240.pdf) shows that a backdoor trigger can be formulated as a subnet and only occupies small portion of net. 
% "Since the backdoor subnet usually only takes a very small capacity of the complete model (less than
% 0.05\% of original capacity in our experiment on VGG16), after it is replaced into the target model,
% the attacked model is expected to still remain its original accuracy on clean input, while present
% adversarial behaviors once the backdoor subnet is activated by backdoor trigger."

\noindent\textbf{Single attacker scenario}
\cite{frankle2018the} showed in their work on the lottery ticket hypothesis that a DNN can be decomposed into a set of subnetworks that carry the same functional similarity and accuracy to the whole DNN. In subsequent works, including MIMO \cite{}, XYZ \cite{}, XYZ \cite{}, we further understand that a subnetwork can be used to represent the set of nodes in a DNN that approximate a sub-function in the DNN that predicts the likelihood a feature pertains to a specific class. Moreover, (https://arxiv.org/pdf/2107.07240.pdf) \cite{} show that a backdoor trigger can be formulated as a subnet and only occupies small portion of a DNN, and that in their work each subnetwork occupied 0.05\% of model capacity. 
Suppose each subnetwork is of a similar or identical size with respect to model capacity (i.e. similar number of parameters).

Suppose we treat the optimization of the parameters $\theta$ of a DNN as a discrete optimization process of subnetworks $\phi$ in $\theta$.
A subnetwork is generally defined to be a subset of nodes within a DNN.
\cite{frankle2018the} formulated the generation of a subnetwork as the nodes on a DNN not zeroed out with a mask $m \in \{ 0,1 \}^{|\theta|}$ and iteratively pruning and optimizing $\theta \odot m$ to identify the minimum required set of nodes to perform inference accurately. 
Moving forward, when we refer to a subnetwork, we refer to an optimal subnetwork $\phi = \theta \odot m$ that is the collection of all pertinent nodes in the DNN for the prediction of a ground-truth class with respect to the set of features, where mask $m$ determines the indices in $\theta$ not zeroed out. In our analysis, there presume the presence of multiple subnetworks, hence multiple masks can co-exist simultaenously and different masks could exist depending on how loss optimization changes $\theta$.
Suppose one optimal subnetwork exists for a unique set of features pertaining to a specific class.
Suppose Stochastic Gradient Descent (SGD) is a sampling procedure that samples $\phi \sim \Phi$. Suppose SGD has optimized $\theta$ with respect to all clean samples already, and the next epoch is considering the insertion of a set of subnetworks with respect to backdoored inputs. 
In this one epoch, we evaluate $\theta_{-1} \rightarrow \theta$ where $\theta_{-1} = \bigcup_{c}^{|\mathbb{D}|} \phi_c$, $\theta = \bigcup_{c}^{|\mathbb{D}|} \phi_c \bigcup \phi_b$ for $|\mathbb{D}|$ inputs:output pairs in the dataset and 1 backdoor trigger.
We denote the poison rate $p = \frac{|X^{\textnormal{poison}}|}{|X^{\textnormal{clean}}| + |X^{\textnormal{poison}}|}$.

We consider loss minimization procedure at this epoch as an implicit measurement of the entropy of the backdoor subnetwork; if there is marginal information:capacity benefit from the insertion of $\phi$ to $\theta$ ($\partial \theta = \phi$) compared to not inserting it, then the subnetwork would be added to $\theta$ in this epoch. 
This update $\theta \rightarrow \theta^{*}$ is represented in equation \ref{equation:0}, where the update condition $\mathcal{L}(\theta \cup \phi^{\textnormal{backdoor}}) < \mathcal{L}(\theta)$ is defined by equation \ref{equation:1}, consisting of loss with respect to both clean and poisoned inputs. 
In-line with our implementation, the loss function is defined by the cross-entropy loss $\mathcal{L}(\theta; x, y) = - \sum_{c}^{|\mathbb{D}|} y_{c} \textnormal{log}(\title{y_{x}})$, which is the cumulative loss for $|\mathbb{D}|$ inputs.
We denote $\textnormal{LHS}$ (\ref{equation:1}) and $\textnormal{RHS}$ (\ref{equation:1}) as the left-hand side and right-hand side of an update condition (\ref{equation:1}) respectively. 
The subnetwork would be updated based on update condition (\ref{equation:1}), where the insertion of the subnetwork would be rejected if $\textnormal{LHS} > \textnormal{RHS}$ (\ref{equation:1}) or $\textnormal{LHS} > \textnormal{RHS}$ (\ref{equation:2}). 
We refactor into update condition (\ref{equation:2}) as a condition: if $\textnormal{LHS} > \textnormal{RHS}$ (\ref{equation:2}), then a subnetwork insertion is rejected.

\begin{equation}
\begin{split}
\theta^{*} := \theta \cup \phi^{\textnormal{backdoor}} \Bigm| \Big\{ \mathcal{L}(\theta \cup \phi^{\textnormal{backdoor}}) < \mathcal{L}(\theta) \Big\}
\end{split}
\label{equation:0}
\end{equation}

\begin{equation}
\begin{split}
& \phantom{X} \mathcal{L}(\theta \cup \phi^{\textnormal{backdoor}}; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \\ & + \mathcal{L}(\theta \cup \phi^{\textnormal{backdoor}}; X^{\textnormal{poison}}, Y^{\textnormal{poison}}) \\ < & \phantom{X} \mathcal{L}(\theta; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \\ & + \mathcal{L}(\theta; X^{\textnormal{poison}}, Y^{\textnormal{poison}})
\end{split}
\label{equation:1}
\end{equation}

\begin{equation}
\begin{split}
& \phantom{X} \mathcal{L}(\theta \cup \phi^{\textnormal{backdoor}}; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \\ & - \mathcal{L}(\theta; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \\ < & \phantom{X} \mathcal{L}(\theta \cup \phi^{\textnormal{backdoor}}; X^{\textnormal{poison}}, Y^{\textnormal{poison}} \\ & - \mathcal{L}(\theta; X^{\textnormal{poison}}, Y^{\textnormal{poison}}) ) 
\end{split}
\label{equation:2}
\end{equation}

\begin{equation}
\begin{split}
\phantom{X} \frac{1}{(1-p)|\mathbb{D}|} \bigg[ & \mathcal{L}(\theta \cup \phi^{\textnormal{backdoor}}; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \\ & - \mathcal{L}(\theta; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \bigg] \\ < \phantom{X} \frac{1}{p|\mathbb{D}|} \bigg[ & \mathcal{L}(\theta \cup \phi^{\textnormal{backdoor}}; X^{\textnormal{poison}}, Y^{\textnormal{poison}}) \\ & - \mathcal{L}(\theta; X^{\textnormal{poison}}, Y^{\textnormal{poison}}) \bigg]
\end{split}
\label{equation:3}
\end{equation}

We refactor into update condition (\ref{equation:3}) to evaluate the average loss (factoring the number of poisoned inputs). Considering the number of poisoned samples affects the information:capacity ratio, if the exclusion of  $\phi^{\textnormal{backdoor}}$ results in complete misclassification of $X^{\textnormal{poison}}$, then for the same capacity requirements, each backdoor subnetwork has a high information:capacity ratio and it is likeley for $\phi^{\textnormal{backdoor}}$ to be accepted. 
In this analysis, the main driving factor for the acceptance of a subnetwork in a single-attacker scenario is the poison rate. 
As the poison rate increases, $\textnormal{RHS}$ (\ref{equation:3}) becomes even larger, and accepts the subnetwork. 
From an existing body of literature on backdoor attacks on DNNs and Figure \ref{fig:multi}($N=10^0$), we know empirically that this condition is satisfied. 

\noindent\textbf{Multiple attacker scenario}
The addition of each backdoor attackers results in a corresponding subnetwork, formulating $\theta = \bigcup_{c}^{|\mathbb{D}|} \phi_c \bigcup \{\phi_{b_n}\}^{N}$ for $N$ attackers.
% The cumulative poison rate $p$ is composed of the poison rates for each attacker $p: \{p_{n}\}^{n \in N}$. 
The cumulative poison rate $p$ is composed of the poison rates for each attacker $p = \sum_n^N p_{n}$. 
Each individual poison rate is thus smaller than the sum of all poison rates, thus the number of backdoored inputs allcoated per backdoor subnetwork is smaller. 
We also presume that any one backdoor poison rate is not greater than the clean dataset, i.e. $(1-p) > p_n \forall n \in N$.
Note that $(1-p)$ includes not only the defender's clean contribution, but also clean inputs contributed by each attacker. 
Given the capacity limitations of a DNN, if the number of attackers $N$ is very large resulting in many candidate subnetworks, not all of them can be inserted into $\theta$.
$\theta$ can only include a fixed number of subnetworks, and this number can depends ultimately by whether 1 subnetwork carries information that can reduce loss for 2 distinct sets of inputs (transferability). We can approximate this transferability by studying how the loss changes with respect to this subnetwork and 2 sets of inputs. There is insufficient results that indicate a precise form of measurement of this transferability in terms of the weight sub-matrice values in the model weights and computing distance scores between subnetworks. 

\begin{equation}
\begin{split}
\frac{1}{(1-p)|\mathbb{D}|} \bigg[ & \mathcal{L}(\theta \cup \{\phi_{n}^{\textnormal{backdoor}}\}^{n \in N}; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \\ - & \mathcal{L}(\theta; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \bigg] \\ <  \sum_{n}^{N} \frac{1}{p_{n}|\mathbb{D}|} \bigg[ & \mathcal{L}(\theta \cup \phi_{n}^{\textnormal{backdoor}}; X_{n}^{\textnormal{poison}}, Y_{n}^{\textnormal{poison}}) \\ - & \mathcal{L}(\theta; X_{n}^{\textnormal{poison}}, Y_{n}^{\textnormal{poison}}) \bigg]
\end{split}
\label{equation:4}
\end{equation}

Another change compared to the single-attacker scenario is that the information:capacity ratio per backdoor subnetwork is diluted. We can infer this from equation \ref{equation:4}, where $N$ subnetworks are required to carry information to compute correct predictions for $p|\mathbb{D}|$ inputs compared to 1 in single-attacker scenario. 
The average loss difference is larger in $\textnormal{LHS}$ (\ref{equation:4}) than $\textnormal{RHS}$ (\ref{equation:4}), hence if it is a question of including all the backdoor subnetworks or none at all, 

\begin{equation}
\frac{\partial \mathcal{L}(X_{g}, Y_{g})}{\partial \theta} \cdot \frac{\partial \mathcal{L}(X_{h}, Y_{h})}{\partial \theta} > 0
\label{equation:5}
\end{equation}

% \begin{equation}
% \mathbb{E}_{X_{g}:Y_{g}, X_{h}:Y_{h} \sim \mathbb{D}}[\frac{\partial \mathcal{L}(X_{g}, Y_{g})}{\partial \theta} \cdot \frac{\partial \mathcal{L}(X_{h}, Y_{h})}{\partial \theta}]
% \label{equation:6}
% \end{equation}

\begin{equation}
\mathbb{E}_{g, h \sim \mathbb{|D|}} \bigg[ \frac{\partial \mathcal{L}(X_{g}, Y_{g})}{\partial \theta} \cdot \frac{\partial \mathcal{L}(X_{h}, Y_{h})}{\partial \theta} \bigg]
\label{equation:6}
\end{equation}

In addition to the magnitude of the change to the loss, we also need to consider the directional change of the loss with respect to each set of subnetworks; in other words, would a selected set of subnetworks reduce the loss on a set of backdoored inputs all in the same direction. We represent this in equation \ref{equation:5}.
$X_{g}:Y_{g}$, $X_{h}:Y_{h}$ are two arbitrary sub-datasets contributed to $\mathbb{D}$ (where $X^{\textnormal{clean}}, X^{\textnormal{poison}} \in \mathbb{D}$); they may be a clean set and a backdoored set, or 2 different backdoored sets. 
Given capacity limitations, every combination of backdoored subnetwork will be evaluated as $\partial \theta = \phi$ against every pair of sub-dataset, and evaluate whether it simultaneously (1) reduces the total loss (Eqt \ref{equation:1}), and (2) returns joint loss reduction with respect to any pair of sub-datasets (Eqt \ref{equation:6}).

\begin{equation}
\begin{split}
& \argmin_{\{ \phi_{k} \} \in \{ \phi_{n}^{\textnormal{backdoor}} \}^{n \in N}} \bigg\{ \frac{1}{(1-p)|\mathbb{D}|} \mathcal{L}(\theta \cup \{\phi_{k}\}; X^{\textnormal{clean}}, Y^{\textnormal{clean}}) \\ & + \sum_{n}^{N} \frac{1}{p_{n}|\mathbb{D}|} \mathcal{L}(\theta \cup \{\phi_{k}\}; X_{n}^{\textnormal{poison}}, Y_{n}^{\textnormal{poison}}) \bigg\}
\end{split}
\label{equation:7}
\end{equation}

The above assumes thus far that only 1 subnetwork can be inserted (when in practice multiple subnetworks may be insertable depending on the transferabiltiy of the candidate subnetworks against the sub-datasets), or that all subnetworks must be inserted or none at all. We extend update condition (\ref{equation:4}) into a subnetwork set optimization procedure (Eqt \ref{equation:7}), where loss optimization attempts to determine a set of backdoor subnetworks that can minimize the total loss over all sub-datasets. 
To make a backdoor subnetwork more salient with respect to procedure (\ref{equation:7}), an attacker could (i) increase their individual $p_n$, (ii) have similar backdoor patterns and target poison labels as other attackers (or any other form of cooperative behavior).
We empirically show this in Experiments \ref{3.4}.

With respect to Experiments \ref{3.3}, adversarial perturbations work because they re-use existing subnetworks in $\theta$ (i.e. $\phi^{\textnormal{clean}}$) without the need to insert a new one.
Stylized perturbations can be decomposed into style and content features; the content features may have transferability against unstylized content features thus there may be no subsequent change to $\phi^{\textnormal{clean}}$, though the insertion of a new $\phi^{\textnormal{style}}$ faces a similar insertion obstacle as $\phi^{\textnormal{backdoor}}$.

To further understand the optimization procedure (Eqt \ref{equation:7}) that obtains the optimal subnetwork set $\{ \phi_{k} \}$, we wish to
approximate the transferability of a subnetwork across sub-datasets and transferability across a set of subnetworks by measuring the distance between a set of class activation maps \cite{}.
Backdoor subnetworks can have varying distances from each other (e.g. depending on how similar the backdoor trigger patterns and corresponding target poison lavels are); to clarify the analysis, we presume that each backdoor subnetwork is distinct for each attacker, and evaluate their distances in our analysis. 

Suppose we retrieve the activations at the $w$th layer of a DNN with parameters $\theta \cup \phi$. We approximate the outputs of the subnetwork as a set of activation values when each input is passed through the weights/biases and then through the activation function (e.g. $\texttt{act} = \texttt{relu}$): $\phi (x) = \{ \{ \texttt{act}(f(\cdot; x, Y_{q})) \}_{d}^{q \in Q} \}^{d \in \mathbb{D}}$ where $Q$ is the number of classes and $x$ is a single input instance in the dataset $\mathbb{D}$. 
We compute an activations set across all classes as a set, and store them all as distinct sets for all inputs in the dataset.
The activations are an indicator of the raw class probabilities; for example, we could retrieve values from the softmax layer.

{\color{blue}{
(https://proceedings.neurips.cc/paper/2018/file/22722a343513ed45f14905eb07621686-Paper.pdf)
Let f(x) denote the function that propagates an input x through the network to the penultimate layer
(before the softmax layer). We call the activations of this layer the feature space representation of the input since it encodes high-level semantic features. Due to the high complexity and nonlinearity of f, it is possible to find an example x that “collides” with the target in feature space, while simultaneously being close to the base instance b in input space by computing

Apparently also do not need to define a dist function, can just say $|| f(x)-f(t) ||_2^{2}$ to indicate distance between them in feature space.
The squared Euclidean norm (squared L2 norm)
% https://www.datacamp.com/community/tutorials/tutorial-machine-learning-basics-norms

}}

Decomposed into class activation maps, we can measure the distance $\texttt{dist}(\phi_{0}(x), \phi_{1}(x))$ between 2 subnetworks by computing a distance score on the same inputs $x$ (constant $x$, varying $\phi$). 
The activation values across all inputs would result in an matrix of dimensions $(|\mathbb{D}|, Q)$. The distance function may be arbitrarily selected, such as a Euclidean distance metric or cosine distance metric; we denote it as $\texttt{dist}(\cdot, \cdot)$ for generality.
This tells us how similar the two subnetworks are, the closer to 0 they are. To return the class activation maps, given that subnetworks can have varying sizes and may not be distinctly able to return uniform dimensions of activations, we presume here that an evaluated subnetwork would be inserted into $\theta$ to make the comparison. 
Measuring the distance between subnetworks would be one way of testing whether a subnetwork carries transferable features for multiple sub-datasets, as at least in the backdoor setting each candidate subnetwork tends to be mapped to a specific sub-dataset. 

Alternatively, we can measure the distance $\texttt{dist}(\phi(x_0), \phi(x_1))$ in the complete set of activations for one subnetwork against all combinations of sub-datasets (varying $x$, constant $\phi$). This would help us approximate the likelihood of a candidate subnetwork reducing loss across a set of sub-datasets. 
Specifically what we would like to show through this decomposition of subnetwork into activations and the measurement of their distance (which the loss comparison equations cannot), is that the collective attack success rates for a set of attackers is dependent on the similarity/overlap of the activations of pixels in an input (backdoor pattern) and the target class labels. 

\begin{equation}
\begin{split}
P \Bigg( & \frac{\partial \mathcal{L}(X_{g}, Y_{g})}{\partial \theta} \cdot \frac{\partial \mathcal{L}(X_{h}, Y_{h})}{\partial \theta} > 0 \bigg| \bigg\{ \\ & \mathcal{L}(\theta \cup \{\phi\}; X_{g,h}, Y_{g,h}) < \mathcal{L}(\theta; X_{g,h}, Y_{g,h}) \bigg\} \Bigg) \\ \propto \frac{1}{|\mathbb{D}|^{2}} & \sum_{g}^{|\mathbb{D}|} \sum_{h}^{|\mathbb{D}|} \texttt{dist}(\phi(X_{g}), \phi(X_{h}))
\end{split}
\label{equation:8}
\end{equation}


{\color{blue}

We address concerns on set-up variations in other sections, in order to determine the root cause of the backfiring effect. Some hypothesis causes are listed here:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Model capacity: \textit{How do we know this backfiring is not attributed to the small capacity relative to 1000 attackers?} We address this in Experiments \ref{} by varying the model capacity, and show that ...
    \item Poison rate: \textit{The poison rate is extremely small in this setup, it is possible the backfiring effect takes place because the target backdoor pattern has not being salient to the model or can be easily ignored by the loss function (Eqt \ref{}) during training?} 
    % In Experiments \ref{}, we do a small-scale study with $N=5$ attackers to show that even with an increase in ------- We have not addressed this, even in coop table, it is still with respect to N=100
    \item Attack configurations: \textit{The poison rate is extremely small in this setup, it is possible the backfiring effect takes place because the target backdoor pattern has not being salient to the model or can be easily ignored by the loss function (Eqt \ref{}) during training? The trigger patterns are randomly generated, how do we know the backfiring effect is not due to a feature collision \ref{NEURIPS2019_7eea1f26} effect between different trigger patterns that are not as dissimilar? The target poison labels are randomly sampled, how do we know the backfiring effect is not due to the collision of similar trigger patterns against dissimilar labels (i.e. a similar pattern but attributed to different labels due to different attackers)? 
    } 
    The poison rate may be small, but we do vary it to different labels in Figure \ref{fig:multi}, and changes across these poison rate indicates that we have surpassed a minimum threshold to measure a backdoor attack (otherwise all the values would have stayed constant regardless of $p$).
    Moreveor in Experiments \ref{}, we do a small-scale study with $N=5$ attackers to show some of these attack configuration changes, including a larger real poison rate per attacker by a magnitude of 2, changes in trigger patterns (including both density of perturbations as well as coordinated orthogonality with respect to other trigger patterns), and changes to target poison labels (where overlap exists to varying extents). 
    
\end{itemize}

}



% \noindent\textbf{Explanation for Experiments \ref{3.1}}
% \noindent\textbf{Explanation for Experiments \ref{3.2}}
% \noindent\textbf{Explanation for Experiments \ref{3.3}}
% \noindent\textbf{Explanation for Experiments \ref{3.4}}
% \noindent\textbf{Explanation for Experiments \ref{3.5}}


==> 4.experiments.tex <==
\section{Evaluation}
\label{4}

% Following up on our understanding of the problem setup and hypotheses, we present our findings on several configuration variations with corresponding explanations.

% \subsection{Methodology}

% \subsection{Evaluation design}

\noindent\textbf{Methodology. }
We implement the baseline backdoor attack algorithm BadNet \citep{8685687} with the adaptation of randomized pixels as unique backdoor trigger patterns per attacker.
% We implement the baseline backdoor attack algorithm BadNet \citep{8685687} with the adaptation that, instead of a single square in the corner, we generate randomized pixels such that each attacker has their own specific trigger pattern (and avoid collisions). 
% We verify these random trigger patterns as being functional for single-agent backdoor attacks at $N=1$. 
% Many existing backdoor implementations in literature, including the default BadNet implementation, propose a static trigger, such as a square in the corner of an image input.
% % , hence for the BadNet algorithm the static pattern does not need to be identical to those used in previous literature (though we do not use this approach for the Clean-label backdoor attack in Experi
% % BadNet requires only variation in the poison rate, which determines the proportion of the dataset to perturb. 
% BadNet only requires a poison rate;
% % In addition to poison rate, 
% we additionally introduce the perturbation rate $\varepsilon$, which determines how much of an image to perturb.
% ;  specifically, for all the pixels available in an image's dimensions, $\varepsilon$ determines how many pixels will be randomly sampled to be perturbed, and randomly sample the degree in which the colour value will change. 
We describe this implementation in Appendix \ref{a1}.
% 
We evaluate upon the CIFAR10 dataset with 10 labels \citep{krizhevsky2009learning}. 
% The poison rate $p$ is the proportion of the \textit{contributed sub-dataset} that is backdoored. 
The real poison rate $\rho$ of an attacker $a_i$ is the proportion of the joint dataset that is backdoored by $a_i$: $\rho = \frac{|X_{i}^{\textnormal{poison}}|}{|\mathbb{D}|}$. 
% (actual number of backdoored samples divided by total number of samples in the joint dataset $|\math|$). 
For $N$ attackers and $V_d$ being the proportion of the dataset allocated to the defender, 
the real poison rate is calculated as  $\rho = (1 - V_d) \times \frac{1}{N} \times p$.
% The allocation of the joint dataset that each attacker is expected to contribute is assumed to be identical (only varying on the number of backdoored inputs); so the collective attacker allocation is $1-V_d$, and the individual attacker allocation is $(1-V_d) \times \frac{1}{N}$.
% Dataset allocations details are discussed in Appendix \ref{a2}.
% As the objective of the backdoor attack is that an attacker wishes to obtain a misclassification when the backdoor trigger pattern is present, and during run-time all samples are poisoned, 
% unless otherwise specified we report accuracy w.r.t. poisoned labels, where a higher value indicates a higher attack success rate.
% The predicted label can be evaluated against either the target poisoned label or the original clean label.
% As the objective of the backdoor attack is that an attacker wishes to obtain a misclassification when the backdoor trigger pattern is present, and during run-time all samples are poisoned, 
% unless otherwise specified we report the run-time accuracy of the predicted labels with respect to (w.r.t.) poisoned labels, where a higher value indicates a higher attack success rate.
% we present the accuracy of the predicted labels with respect to the poisoned labels, where a higher value indicates a higher attack success rate.
% To measure a collective attack success rate, we present the mean and standard deviation of the accuracy w.r.t. labels for each attacker's run-time set $\texttt{mean} \pm \texttt{std}$.
% In Figures, accuracy is out of 1.0; in Tables, accuracy is out of 100.0.
% We elaborate on the distinction between train-time and test/run-time sets, as well as dataset allocations in Figure \ref{fig:allocation} (Appendix \ref{a2}).
% Run-time is denoted as the inference period upon which the model trained and validated on a dataset pool will make predictions on backdoored inputs. 
% We visualize the dataset allocation in Figure \ref{fig:allocation} (Appendix \ref{}).
% 
% The distribution of target poison labels may or may not be random.
% The distribution of clean labels are random, as we randomly sample inputs from the attacker's private dataset to re-assign clean labels to target poison labels.
% As all our evaluation datasets have 10 classes, this means $\frac{1}{10}$ of all backdoored inputs have target poison labels equivalent to clean labels.
% % Hence, the lower bound for both Attack Success Rate (accuracy w.r.t. poisoned labels) and Standard Accuracy (accuracy w.r.t. clean labels) are both 0.1.
% We only tabulate the raw accuracy w.r.t. poisoned labels;
% a more reflective attack success rate would be ($\texttt{Acc w.r.t. poisoned labels}-0.1$).
% 
% As the sampling of inputs for assignment of the poisoned label is random, it would be expected that $1/10$ of inputs had been assigned poisoned labels that were identical to their clean labels, so an accuracy w.r.t. poisoned labels above 0.1 is favorable for individual attackers.
% An accuracy below 0.1 could arise either because of randomness in clean label allocation (e.g. in one instance, there is only 0.09 inputs where clean labels coincide with poison labels) or the accuracy of the model on clean inputs has dropped and clean-labeled inputs were also misclassified. 
% 
% We summarize the main experimental conditions in this section; more details can be found in Appendix \ref{a2}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Multi-Agent Attack Success Rate}
\label{3.1}
% poison rate vs epsilon (vs num attackers)

\input{tables/multi_agent}

In this section, we investigate the research question: what effect on attack success rate does the inclusion of an additional attacker make? 
The base experimental configurations (unless otherwise specified) are listed here and Appendix \ref{a2}.
% To validate this, we detail as follows the experimental configurations adopted to demonstrate the multi-agent backdoor attack. There are also the base experimental configuration for other experiments (unless otherwise specified).
$V_d = 0.1$, and target poison label for each attacker is randomly selected. 
Results are summarized in Figure \ref{fig:multi}.

% \noindent\textbf{Attacker configurations. }
% We acknowledge that a decrease in number of attackers can result in more of the dataset pool available for poisoning, and this can result in a larger absolute number of poisoned samples if the poison rate stays constant. To counter this effect, we take into account the maximum number of attackers we wish to evaluate for this experiment, $N=1000$, such that even as $N$ varies, the real poison rate per attacker stays constant. 
% In this case, as we wish to test a large number of attackers $N=1000$ with small poison rates $p=0.1$ for completeness, we set the defender allocation to be small $V_d=0.1$. This allocation gives sufficient space for 1000 attackers, and we also verify that this extremely poison rate can still manifest a, albeit weakened, backdoor attack at $N=1$. 
% $V_d=0.1$; 
% The run-time poison rate is 1.0 (all run-time $X^{\textnormal{poison}}$ are backdoored). 
% % \item 
% For each $x^{\textnormal{poison}} \in X^{\textnormal{poison}}$, 
% each attacker randomly samples a target poison label out of 10 classes. 
% The trigger label is the label that the triggered input should carry. 
% In a clean label attack, the trigger label would be the original label, and the trigger pattern would applied to this cleanly-labelled image. 
% No information sharing or cooperation is presumed.
% \item We assume absolutely no coordination here: randomly selected triggers, no coordinated trigger pattern selection, etc.
% \item 
% For ASR evaluation, the 20\% run-time split set of each attacker has a run-time poison rate of 1.0 (i.e. the whole run-time set is poisoned with the same backdoor trigger patterns as used in train-time).
% \end{itemize}

% \noindent\textbf{Defender configurations. }
% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
%     \item 

% and total dataset size of 60,000
% \item 
% We trained a ResNet-18 \citep{He2015} model with batch size 128 and with early stopping when loss converges (approximately $30$ epochs, validation accuracy of $92-93\%$; loss convergence depends on pooled dataset structure and number of attackers).
% We use early-stopping for a large number of epochs, as this training scheme would be reused and ensures consistent loss convergence given varying training datasets (e.g. training a model on augmented dataset with backdoor adversarial training, training a model on 
% We use a Stochastic Gradient Descent optimizer with $0.001$ learning rate and $0.9$ momentum, and cross entropy loss function.
% \item 
    
% \end{itemize}

\noindent\textbf{(Observation 1: Failed multi-agent backdoor attack)}
% \noindent\textbf{Findings. }
% Results are summarized in Figure \ref{fig:multi}.
As $N$ increases, the accuracy w.r.t. poisoned labels for $(p, \varepsilon)$ tends to decrease, and converges at 0.1.
% We learn that as $N$ increases, the accuracy w.r.t. poisoned labels for $(p, \varepsilon)$ tends to decrease, through at $N=100, 1000$ the values do not change much, which possibly is indicative of a convergence of accuracy drop, given that the accuracy is around 0.1.
% ; this convergence is consistent across other experiments.
% we evaluate this the convergence with respect to capacity in Experiments \ref{}.
% We learn that for each $p$ holding $\varepsilon$ constant (and vice versa), the accuracy w.r.t. poisoned labels continues to decrease until $N=10$; at $N=100, 1000$ we observe that the accuracy stays constant and is agnostic to $p, \varepsilon$ at this point. 
For every $N$, at each $\varepsilon$ the standard deviation of accuracy is similar;
% stays at a similar level; 
however, as $\varepsilon$ increases at each $p$, the standard deviation also increases, i.e. anti-correlation between the mean and standard deviation.
We denote the phenomenon as the \textit{backfiring effect}, where the introduction of additional attackers reduces the importance of the presence of the trigger in performing a backdoor attack.
% This occurs regardless of dataset, model capacity, poison rate, trigger pattern generation, target poison label selection, optional use of backdoor defense, agent cooperation, or other joint distribution shift perturbations.

% In corroboration with findings in subsequent experiments, 
% we denote this phenomenon as the \textit{backfiring effect}, where the introduction of additional attackers reduces the importance of the presence of the trigger in performing a backdoor attack.
% This occurs regardless of dataset, model capacity, poison rate, trigger pattern generation, target poison label selection, optional use of backdoor defense, agent cooperation, or other joint distribution shift perturbations.
% A primary advantage of the backfiring effect is that it presents itself as a natural defense against multi-agent backdoor attacks.
% Existing models do not necessarily need to interfere too severely with their models in consideration of multi-agent backdoor attacks (though if there are other trade-offs, this will need to be studied as future work). 
% It motivates backdoor defenses in practical settings, as most backdoor defenses are directed to single-attacker setups, but if it is likely that multiple attackers can exist, then the defender can focus on other aspects of model robustness other than backdoor robustness. 

% * We measure the real or absolute poison rate, not nominal poison rate - this means, we need to limit each poison rate by what is the max proportion of the dataset any one attacker can contribute (example: it does not make sense that every attacker can contribute 1.0 dataset).
% * This set of charts assume constant poison rate across all attackers
% * Actual way of calculating the poison rate is (1 - defender_fracs) * 1/N * poison_rate
% * Assume absolutely no coordination here: randomly selected triggers, no trigger pattern selection etc; just assume constant poison limit and constant epsilon
% * Important insight: this table tells us how Collective ASR varies with poison rate, epsilon BUT ALSO RANDOMNESS IN TRIGGER SELECTION -- when epsilon = 0 and poison rate = 0, during run-time the trigger selection is still random (i.e. trigger assignment still occurs) but run-time poison rate is 1.0 -- in other words, we can observe the marginal ASR differences with respect to poison/epsilon and not just trigger selection
% * Having normalized/baselined for the randomness of trigger selection and its adversarial impact on collective ASR, we can see a linear relationship, where an increase in poison rate and epsilon will lead to greater variance of ASR, while also letting some attackers maximize their own individual ASR
% * Translated into Collective ASR: min, mean +/- std, max
% * p=0 scenario does not seem right at all, esp when an attacker has ASR=1.0… this will make a reviewer suspect we have a bug, it may be best to remove this
% * Observation: though the collective ASR has increased, we note that the clean-label acc per attack is slighlty higher than poisoned acc, though not that high…what this indicates, is that though backdoor attackers failed to backdoor, they did succeed in poisoning (unless we try to increase the epoch count?)
% * Put in explanations for anomalous values / caveats etc


% \myp{Varying poison rate $p$.} In the first scenario (Table \ref{single1}), we evaluate the multi-agent attack success rates with respect to a change in poison rate. 
% (1) We first hold the poison rate constant, and show a drop in attack success rate for each attacker as soon as multiple attackers with the same poison rate are introduced.
% % When the number of attackers increases, the ASR for all the attackers fall compared to if they attacked alone, further corroborated in Table \ref{single2}. 
% We refer to this as the \textbf{\textit{backfiring effect}}, where the introduction of additional attackers reduces the importance of the presence of the trigger.
% (2) We then analyze what happens when attackers increase their individual $p$, increasing the aggressiveness of their attack.
% % other forms of aggression include the use of counter-triggers (the generation of trigger patterns that are intentionally meant to backfire other attacker's patterns), or develop novel backdoor trigger patterns unknown to any other attacker.
% Unsurprinsingly, when a single attacker increases their own $p$, ASR improves for the aggressor and weakens for the others.
% % When there are multiple attackers with varying levels of aggressivity in their attack parameters, in the case that an attacker is more aggressive with their backdoor inputs, they can still maximize their ASR relative to other attackers, and keeps others' scores even lower; however, it leads to mutually-assured destruction of attack success rate of all attackers when all attackers use the maximum available parameter settings. 
% (3) When all the attackers escalate their poison rate, they all weaken their ASR collectively.
% Once attackers start to escalate or aggressively poison the dataset to gain significant attack success rate, they collectively achieve what we might refer to as \textit{mutually assured destruction (MAD)}. 
% The perturbations are no longer imperceptible (e.g. could be detected by clustering methods). 
% If we introduce different variations (e.g. different poison rate, identical triggers), the change in attack success rate may be uneven between the attackers, but in general there is a significant drop in each of their attack success rates compared to before they performed the attack. 
% % , blocked by multi-agent defenses, etc
% % They all achieve the same poor accuracy as if they did not escalate at all. 
% Collaboration cannot be taken as an assumed workaround, as any attempt to attack the attack success rate of other attackers requires either novel techniques (which would be eventually known by others, and this arbitrage is nullified when number of attackers tend to action set) or increasing attack aggressiveness (which is shown to lead to MAD).
% Cooperation may not resolve this scenario either, as betraying cooperating agents may favour ndividual agents, thus even in a cooperating environment each attacker in attempting to maximize their personal ASR would minimize the collective ASR. 


% \myp{Varying trigger label.} In the second scenario (Table \ref{single2}), we vary the trigger label. 
% (1) We first hold the trigger labels all constant. As all the attackers are aiming for the same target class, they are all mutually diluting the saliency of their respective trigger pattern in the distribution of salient features for that target class. 
% % and show that there is conflicting saliency in features for the same label.
% (2) We then have each attacker having a distinctly different label. The ASR is still lower than if they were individual attackers. 

% Adjusting the poison rate and trigger label has demonstrated that changing the distribution of features salient to the target class is the main cause for a loss in ASR for attackers in a multi-agent setting. Using the same label introduces additional features paired to the target class, and increasing the poison rate broadens the distribution of features. 
% We observe that the incorporation of multiple attackers in itself acts as a \textit{natural} defense against multi-agent backdoor attacks, hence there is utility in finding properties that can be transferred so as to construct defenses.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Game variations}
\label{3.2}

In this section, we wish to investigate: do changes to the game setup (action-independent variables) manifest different effects in the multi-agent backdoor attack? 
% In subsequent sections, we will specifically investigate alterations in the actions taken by agents, but in this section we instead focus on alterations in variables that is assumed to be out of the control of attackers and defenders and constant with respect to the payoff functions, specifically focusing on model capacity and source dataset. 
$V_d = 0.2$, $\varepsilon, p = 0.55$, and target poison label for each attacker is randomly selected. 
Results are summarized in Table \ref{tab:dataset1} and Figure \ref{tab:capacity}. 

% With respect to attacker configurations, $V_d = 0.2$, backdoor perturbation rate $\varepsilon$ at $0.55$, train-time poison rate at $0.55$,
% % (real poison rate per attacker $0.0044$), 
% run-time poison rate at $1.0$, and target poison label for each attacker is randomly selected. 
% % All other attack configurations are identical to that in Experiments \ref{3.1}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Dataset}
We use 4 datasets, 2 being domain-adapted variants of the other 2. MNIST \citep{lecun-mnisthandwrittendigit-2010} and SVNH \citep{37648} are a domain pair for digits. CIFAR10 \citep{krizhevsky2009learning} and STL10 \citep{pmlr-v15-coates11a} are a domain pair for objects.
% We make use of the whole dataset instead of the pre-defined train-test splits provisioned, given that we would like to retain custom train-test splits for defenders and also because we have an additional run-time evaluation set for attackers (Figure \ref{fig:allocation}). 

\input{tables/dataset}

% * Need to explain why we are considering clean-label acc; we set run-time poison rate to 1.0, and we want to put into perspective which labels that were triggered also happened to be clean; we also want to show that the clean acc did not surpass poison
% * 2 ways we can spin the CIFAR10 weak performance for N=1 being less than 9x% - either we used this as the weakest performing baseline across all datasets, OR we push its values up by re-running
% * Place the clean validation acc in appendix as part of training procedure?

% ^MNIST is a problem double check this

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Capacity}
For capacity variations, we trained with the same training procedure as Experiments \ref{3.1} with varying model architecture:
SmallCNN (channels $[16,32,32]$) \citep{fort2020deep},
ResNet-\{9, 18, 34, 50, 101, 152\} \citep{He2015},
Wide ResNet-\{50, 101\}-2 \citep{BMVC2016_87},
VGG 11-layer model (with batch normalization) \citep{Simonyan15}.
% Due to computational constraints, we wished to sample number of attackers $N$ for the following ranges ($1…10$,	$10…20$, $20…100$, $100..500$,	$500…1000$), linearly-spaced these ranges into 3 segments, and evaluated on all the returned $N$. 
% For Wide ResNet, the model is the same as ResNet except for the bottleneck number of channels which is twice larger in every block. The number of channels in outer 1x1 convolutions is the same, e.g. last block in ResNet-50 has 2048-512-2048 channels, and in Wide ResNet-50-2 has 2048-1024-2048.
% Other than ResNet, we included other architectures including VGG11 (a comparably large capacity model to Wide ResNet-101 in terms of number of parameters but with different architecture) and SmallCNN (a small capacity model used in recent loss landscape analysis literature).

\input{tables/capacity}

% * A convergence effect is observed, where they all converge to about mean 0.10
% * Exact same attack config and training config; same poison rate, same eps, same epochs, so it makes sense that N=1 ASR goes down as capacity goes up
% * (https://arxiv.org/pdf/2010.14495.pdf) shows that wider network width for same capacity should have better accuracy improvements than less wide for same capacity (measured as number of parameters)	
% * Doesn't make sense, it appears they all converged at the same rate, regardless of model complexity	
% 	* In-line with (https://arxiv.org/pdf/1906.00830.pdf) and our own table for N=1, we learn that the backdoor attack is relatively capacity-agnostic, in other words even large capacity models can learn a trigger pattern; the explanation on why they converge similarly has less to do with model capacity and more to do with number of attackers, as is in a single attacker case
% * Process for OOM of N=1: we first trained on 10% defender_fracs, exported weights, set overwrite=False, then set defender_fracs to 80% and evaluate on attacker_train_set 20% --> the model is still trained on a limited 10% poisoned set, just the eval set is constant (plus trigger is constant cuz of seeding)	
% 	* resnet152 at n=1 is a funky outlier eh

% \noindent\textbf{Findings. }
\noindent\textbf{(Observation 1 cont'd)}
% Results are summarized in Table \ref{tab:dataset1} and Figure \ref{tab:capacity}. 
As we vary by datasets, we observe consistent patterns of successful single-agent backdoor attacks
% (with high accuracy w.r.t. poisoned labels) 
as well as unsuccessful multi-agent backdoor attacks. 
In addition, across all these datasets, the drop in the defender's validation set accuracy (with respect to clean labels for unpoisoned inputs and poisoned labels for poisoned labels) between $N=1$ to $N=100$ is close to negligible (with slight drop for STL10).
Most of the attacker allocation was allocated to run-time than train-time, hence the defender validation accuracy faced minimal impact with respect to the reduction in poisoned label accuracy. 

\noindent\textbf{(Observation 2: Collective payoff convergence)}
Mean run-time accuracy w.r.t. both poisoned and clean inputs tend to converge towards 0.1.
% In both attacker count cases, the run-time accuracy w.r.t. both poisoned and clean inputs tend towards 0.1. 
% With model variations, as the number of attackers increase, a general convergence to approximate mean accuracy w.r.t. poisoned labels of 0.10 is observed. 
% For poisoned labels, this can be explained by the overlapping case where a poisoned label is identical to the clean label for a randomly sampled input. For clean labels, this can be explained as random guessing by the model across 10 classes.  

\noindent\textbf{(Observation 3: Low accuracy w.r.t. clean labels with trigger)}
One visible downside of the multi-agent backdoor attack presented here, and consistent with experiment results in other sections, is the low clean label accuracy when poison rate = 1.0. Though the backdoor attack's primary objective has failed for the attackers (maximizing accuracy w.r.t. poisoned labels), the attackers successfully poison the model into make faulty predictions, and even the use of backdoor defenses cannot retain clean label accuracy.

\noindent\textbf{(Observation 3: Independent from model capacity)}
% As to model variations, as the number of attackers increase, a general convergence to approximate mean accuracy w.r.t. poisoned labels of 0.10 is observed. 
In-line with \cite{10.1145/3474085.3475591} and our own table for $N=1$, we learn that a single-agent backdoor attack is capacity-agnostic, where even large capacity models can be backdoored and learn trigger patterns. 
At $N=1$, there is an inverse pattern where the larger the model capacity, the lower the accuracy w.r.t. poisoned labels. This is in-line with \cite{}, where we would expect a larger poison rate would be needed to render a subnetwork in a larger capacity model. 
Our expectation would be that for larger capacity models, they would be able to retain more backdoor subnetworks of multiple agents. However this is not the case: even as small as 5 attackers, we find that the mean accuracy for all models has already fallen to below 0.4, and there is a consistent decline for both the mean and standard deviation, where the values are similar across all models at each $N$. 


% (https://arxiv.org/pdf/2010.14495.pdf) shows that wider network width for same capacity should have better accuracy improvements than less wide for same capacity (measured as number of parameters)	
% Doesn't make sense, it appears they all converged at the same rate, regardless of model complexity	
% In-line with (https://arxiv.org/pdf/1906.00830.pdf) and our own table for N=1, we learn that the backdoor attack is relatively capacity-agnostic, in other words even large capacity models can learn a trigger pattern; the explanation on why they converge similarly has less to do with model capacity and more to do with number of attackers, as is in a single attacker case

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Changes in model parameters}
% \label{3.6}

% \begin{figure*}[]
%     \centering
%     \includegraphics[width=\textwidth]{assets/cos_dist.pdf}
%     \includegraphics[width=1.02\textwidth]{assets/cos_dist_colorbar.pdf}
%     \caption{}
%     \label{fig:cos_dist_subnet}
% \end{figure*}

% In this section, we wish to understand how the parameters of the model change as the number of attackers increase.
% We wish to explore our subnetwork analysis empirically to observe whether our hypotheses are reflected in changes in model parameters.
% To measure a likelihood that a set of trained models on different attack configurations contain similar subnetworks, in this setting we measure the distance in parameters, specifically the distance in parameters per layer for the full original DNN, as well as the distance in parameters per layer in a pruned DNN.
% Results are summarized in Figure \ref{fig:cos_dist_subnet}. 

% Other than $\varepsilon, p = 0.55$ and training SmallCNN, 
% we retain the same attacker/defender configurations as Experiments \ref{3.1}.
% % , with the exclusion of the defender's model being the SmallCNN architecture. 
% We adopt SmallCNN for its low parameter count, which would be helpful in simplifying the subnetwork generation and analysis, as well as overall interpretability. 
% In addition, as we show that the backdoor attack is consistent across all model architectures (Experiments \ref{3.2}), using a smaller model means the subnetworks with respect to the complete network is less diluted and larger in proportion (and hence the cosine distance would be less diluted for our observation). 
% % Explain why SmallCNN
% % Explain why not using feature space visualization
% % Explain why not using subspace movement plot

% We start with a fixed random initialization, shared across the 4 models trained on $N$ = 1, 10, 100, 1000.
% We use \cite{frankle2019lottery}'s Iterative Magnitude Pruning (IMP) procedure to generate a pruned DNN (0.8\% in size of the full DNN across all $N$s), also denoted as the lottery ticket. The lottery ticket is a subnetwork, specifically the set of nodes in the full DNN that are sufficient for inference at a similar performance as the unpruned DNN.
% The study of the lottery ticket helps us make some inferences with respect to how the feature space changes, as well as where the optima on the loss landscape has deviated.
% We compute the cosine distance per layer between (i) parameters in the full DNN, (ii) mask of the lottery ticket against the DNN, (iii) parameters of the lottery ticket.
% We plot the values of $N$ v.s. $N$ for the weights and biases matrices for each convolutional layer ($\texttt{conv2d\{layer_index\}}$) and fully-connected layer ($\texttt{fc\{layer_index\}}$).
% All in all, the lottery ticket is a proxy for the most salient features, hence also acts as an alternate feature space representation.

% % Argument on why we use compare w.r.t. pruned networks:
% % Each time we insert a new agent / trigger pattern, even with const rand init, the rest of the layers change drastically w.r.t. SGD, so it would be expected that each subnet:DNN optimization procedure would be starkly different;
% % Instead, we evaluate the pruned network, both the mask as well as the whole weights -- the size should be increasing over time since there are 100 triggers (if not, that's a problem), and the mask overlap should be comparable (at least per layer)
% % Warnings:
% % - in IMP, we set the criteria on how small the network should be, so it's not a strong argument to compare size -- alternatively, we want to show the change in cosine distance of the pruned network with respect to constant capacity reduction (it is sort of a proxy for most salient feature capture)
% % - To compute cosine distance, we compute for each 2 matrix (norm 2 etc), and we flatten them out layer by layer
% % - We use small scale model, as per other papers on loss landscape analysis, hence we use SmallCNN
% % IGNORE (we did not do this) - we exclude some layers: we definitely excluded softmax layer -- layers: input layer, fc layer, pooling layer, softmax layer, output layer
% % We preserve the positional indices of the params: instead of only returning non-zeroed param values, we directly multiplied the one-zero mask against the params so position is retained
% % - We do the pruning to reduce dimensionality from 15,722 to 126, 126-dimensions
% % - We start with constant rand init --- VERY IMPORTANT

% % nn.Conv2d is used to define the convolutional layers. We define the channels they receive and how much should they return along with the kernel size. We start from 3 channels, as we are using RGB images
% % nn.MaxPool2d is a max-pooling layer that just requires the kernel size and the stride
% % nn.Linear is the fully connected layer, and nn.ReLU is the activation function used
% % https://discuss.pytorch.org/t/understanding-model-parameters/68783/2

% \noindent\textbf{(Observation 4: Increasingly-distant model parameters)}
% % \noindent\textbf{Findings. }
% We make the following observations:
% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
%     \item The values of the biases for most layers have not changed significantly and fall under the distance region $0.0 - 0.1$. 
%     \item For the first convolutional layer ($\texttt{Conv2d0}$) weights, 
%     we observe that the weights change significantly as soon as an additional attacker is introduced: the weights for $N=10, 100, 1000$ are closer to each other, and only $N=1$ has a distinctly large distance from all others.
%     This returns an implication that the saliency reduction effect is immediate, and the tradeoff between ASR and number of attackers occurs as soon as the number of backdoor trigger patterns is more than 1. 
%     In addition, it does not indicate a significant diminishing marginal effect, where the weights distance change is significant with respect to an increase in attackers. 
%     \item The pattern for $\texttt{Conv2d0}$ is exacerbated in $\texttt{Conv2d1}$ and $\texttt{Conv2d2}$.
%     There is a very clear trend, where although the distance reduction is not as linear in $\texttt{Conv2d0}$, it is clearly linear the further we go down the layers in the network, where: for the weights of a layer for 2 different models trained under 2 distinct attacker configurations (different $N_0$, $N_1$), the further that $N_0$ and $N_1$ are jointly distant from 1, the closer their cosine distance is. The further down the convolutional layer indices we evaluate, the distance differentials become more stark and distinct. 
%     \item We observe that the distance patterns for the cosine distance with respect to the full network parameters, mask of the lottery ticket, and parameters of the lottery ticket are all extremely similar: this implies to us that the main driving changes to the optima computed (and the main driver for the distance between weights in the full network) is specifically attributed to the changes in the lottery ticket required to resolve the backdoor trigger pattern. It follows through on our previous analysis, that the main driving factor for the DNN optimization is the insertion or rejection of a subnetwork.
%     \item For all the fully-convolution layers (weights as well as biases), we observe a pattern where the lottery ticket drives the distance outcomes across all 3 cosine distance matrices.
%     We also observe an asymmetrical pattern compared to the convolutional layers, where the further down the fully-connected layer indices we evaluate, the distance differentials become less stark. In earlier $\texttt{fc}$ layers, there is a similar pattern to the $\texttt{Conv2d}$ layers, where the further that $N_0$ and $N_1$ are jointly distant from 1, the closer their cosine distance is. 
% \end{itemize}
% % Now we need some theoretical explanations, something more than just reading out the charts


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \subsection{Joint shift: label and domain}
\subsection{Additional shift sources}
\label{3.3}

The multi-agent backdoor attack thus far manifests joint distribution shift in terms of increasing variations per source; how would it manifest if we increases sources?
% In other Experiments, joint distribution shift takes place with respect to multiple label shifts taking place at train-time, specifically through the use of multiple backdoor triggers. 
% Here, we are interested in studying the joint distribution shift between multiple perturbation sources, evaluating an $N>1$ setting where we have $1-3$ distinct sets of perturbations of varying quantity against an $N=1$ setting where we have 3 distinct sets of perturbations of 1 quantity each or an $N>1$ setting where we only have backdoor perturbations of varying quantity. 
% We retain the defender configurations from Experiments \ref{3.1}.
Adversarial perturbations, introduced during test-time, are generated with the Fast Gradient Sign Method (FGSM) \citep{goodfellow2015explaining}.
Stylistic perturbations, introduced during train-time $\alpha = 1.0$  means 100\% stylization, are generated with Adaptive Instance Normalization
(AdaIN)\citep{huang2017adain}.
Further evaluation details in Appendix \ref{a3.3}.
% If the target poison label is non-identical to the clean label, then both a backdoor attack and adversarial attack will succeed in rendering a misclassification w.r.t. clean labels, i.e. 
% the attack objective of the attacker is to minimize the accuracy w.r.t. clean labels. 
Results are summarized in Figure \ref{fig:joint_1} and Figure \ref{fig:joint}. 
% In this section, we consider the complete range of values of $\alpha$, where to save space the remaining results for $\alpha=0.5$ are found in Figure \ref{fig:joint} (Appendix \ref{}).

% \input{tables/joint_shift}

% Attacker configurations:

% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    
    % \item 
% For adversarial perturbations, we use the Fast Gradient Sign Method (FGSM) \citep{goodfellow2015explaining}. 
% With this attack method, adversarial perturbation rate $\varepsilon_{\textnormal{adv}}=0.1$ can sufficiently bring down the attack success rate comparable and similar to that of $\varepsilon_{\textnormal{adv}}=1.0$; we do this to induce variance. Hence, we scale the perturbation against an upper limit $1.0$ in our experiments, i.e. $\varepsilon_{\textnormal{adv}}^{'} = 0.1 \times \varepsilon_{\textnormal{adv}}$.
% Argue that actual epsilon E is sufficient to bring ASR down to 0, so we scale the Adv eps as a fraction of E; e.g. if Eps=25 == Eps=255, then instead we compute eps=0.1*25…1.0*25		
% Adversarial perturbations, introduced during test-time, are generated with the Fast Gradient Sign Method (FGSM) \citep{goodfellow2015explaining}, where each attacker only crafts adversarial perturbations with respect to their own private dataset (i.e. they train their own surrogate models with the same training scheme as the defender, and do not have any access to the joint dataset to craft perturbations).
% It is also worth noting that FGSM computes perturbations with respect to the gradients of the attacker's surrogate model where this model was trained on the attacker's private dataset, which contains backdoored inputs mapped to poisoned labels, meaning the feature representation space is perturbed with respect to backdoor trigger patterns. 
% We do not train a surrogate model with respect to the clean private dataset, as the intention of a surrogate model is to approximate the target defender's model which has been assumed to be poisoned, and it is also in the attacker's best interests to introduce adversarial perturbations even with respect to the backdoor perturbations, as long as a misclassification occurs (which we can verify with the clean-label accuracy). 

    % \item 
% For stylistic perturbations, we use the Adaptive Instance Normalization
% (AdaIN) stylization method \citep{huang2017adain}, which is a standard method to stylize datasets such as stylized-ImageNet \citep{geirhos2018imagenettrained}.
% Dataset stylization is considered as texture shift or domain shift in different literature. 
% We randomly sample a distinct (non-repeating) style for each attacker.
% $\alpha$ is the degree of stylization to apply; 1.0 means 100\% stylization, 0\% means no stylization.
% We follow the implementation in \cite{huang2017adain} and \cite{geirhos2018imagenettrained} and stylize CIFAR-10 with the Paintings by Numbers style dataset. We adapt the method for our attack, by first randomly sampling a distinct set of styles for each attacker, and stylizing each attacker's sub-dataset before the insertion of backdoor or adversarial perturbations. This shift also contributes to the realistic scenario that different agents may have shifted datasets given heterogenous sources. 
% We present the values for $\alpha=1.0$, in accordance with \cite{geirhos2018imagenettrained} for stylize-ImageNet, but also present the numbers for $\alpha=0.5$ in Figure \ref{fig:joint}. 
    
    % * It's interesting to see that ASR is higher when either max or min stylization, but not in between!	
    % * Clarify definition of poison rate: proportion of dataset allocated to attacker contribution that is poisoned (i.e. p*(1-def_fracs))	
    % * Style alpha = 0 is the equivalent of no style transfer; in other words, the third table includes both eps_adv vs eps_backdoor (at style=0) as well as eps_adv-eps_backdoor vs style	

    % * According to "feat = feat * alpha + content_f * (1 - alpha)", alpha 1.0 means NO content_f
    % alpha is how much stylization to apply; 1.0 means 100% stylization, 0% means no stylization
    
    % Stylization alpha = 0 : No stylization
    % Warning: We use only 0.1 subset of CIFAR10		

    % \item 
% The defender allocation is set to 0.5. For all other attack variables, we retain the attacker configurations from Experiments \ref{3.1}.
% Other than $V_d = 0.5$, all other attacker configurations are retained from Experiments \ref{3.1}.
% The defender allocation is set to 0.5. For all other attack variables, we retain the attacker configurations from Experiments \ref{3.1}.
% > It would be very helpful to add a row in all tables indicating real_poison_rate --- warning, the real poison rate is even lower, re-read logs, it is not 0.24, it is around 0.05 even for poison rate 0.8
% List out the real_poison_rate in the text/label with explanation: 					0	0.0401	0.0796	0.1618	0.1988
% For first 5 rows of cont'd table, we re-use poisonrate=0.0 values since it is meaningless for backdoor_eps=0.0 with poisitve poison rate	
% When the poison rate is 0.0, then the accuracy w.r.t. poisoned labels is equivalent to the accuracy w.r.t. clean labels. 
% In our results, target poisoned labels are the intended labels based on attacker preferences, being clean labels for clean untriggered inputs and poisoned labels for backdoor triggered inputs. 
% This means that when the run-time poison rate is 0.0, then the accuracy w.r.t. poison and clean labels are identical (we also show the values for both separately in Figure \ref{fig:joint} anyways). 
% It also means that when $\varepsilon, p = 0.0$, then this set of values would be identical for accuracy w.r.t. poison as well as clean labels. 
    
% \end{itemize}

% Prior to interpreting the results, we need to consider the attack objective of the attacker. For a backdoor attack, an attacker's objective is to maximize the accuracy w.r.t. poisoned labels. In an adversarial attack, an attacker's objective is to minimize the accuracy w.r.t. clean labels. The attack objectives may have additional conditions in literature, such as imperceptability to humans, or retaining high accuracy on clean inputs, etc, but the aforementioned 2 are the primary goals. 
% They may not necessarily be contradictory either for two reasons:
% (i) if the poisoned label is non-identical to the clean label, then both a backdoor attack and adversarial attack will succeed in rendering a misclassification w.r.t. clean labels; and (ii) one similarity between a backdoor attack and adversarial attack is that they both rely on varying fidelity of information of the train-time distributions, where the backdoor attack has white-box knowledge of the perturbations that will cross the decision boundary to a target class, while the adversarial attack has grey/black-box knowledge of perturbations that may have a likelihood of crossing the decision boundary to a target class.
% We further elaborate on (ii) in Appendix \ref{a1}.
% In any case, we conclude for this evaluation that the attack objective of the attacker is to minimize the accuracy w.r.t. clean labels. 

% \noindent\textbf{Findings. }
% Results are summarized in Figure \ref{fig:joint_1}. 
% In this section, we consider the complete range of values of $\alpha$, where to save space the remaining results for $\alpha=0.5$ are found in Figure \ref{fig:joint} (Appendix \ref{}).

{\color{blue}
Suspicious: the clean label accuracy did not from when stylization is introduced?
could we argue it is because of the early stopping mechanism?
}


First, we evaluate the shift combination of \{backdoor, stylized\}.
This is an evaluation of distinctly train-time perturbations. 

\noindent\textbf{(Observation 3 cont'd)}
Referencing the value sets for run-time poison rate 0.0 (backdoor poisoned, but trigger not activated), 
one interesting phenomenon we would like to point out is that the accuracy w.r.t. clean labels is low \textit{only when the backdoor trigger is present}; when the backdoor trigger is \textit{not} present, be it $N=1,100$ or $\alpha=0.0, 1.0$, a high clean label accuracy is retained, as high as a model trained on a dataset with no backdoor attack at all. 
This is important to note, as this mean the multi-agent backdoor attack does \textit{not} violate the secondary objective of the attacker, which is that the backdoor attack does not affect standard performance on clean inputs. 

\noindent\textbf{(Observation 1 cont'd)}
Referencing the value sets for run-time poison rate 1.0 (poisoned and activated), at $N=1$ the stylized perturbations do not appear to make a significant change to the attack success rate (possibly as the ASR is already bounded by 0.1),
which informs us that the joint shift between a backdoor trigger pattern and input style do not manifest a joint-saliency effect, where one shift reinforces the saliency of the other during test-time. This would make sense, given that this style would be present in inputs of other classes (including unpoisoned inputs); this effect likely manifests if the stylization is applied to poisoned inputs only. 
To the contrary, 
in the $N=100$ setting we find that the introduction of stylized perturbations indeed contributes to a further decrease in attack success rate, particularly at high $\varepsilon_{\textnormal{b}}, p$. A shift in texture/style between attackers contribute to the backfiring effect, reaffirming the hypothesis that a joint distribution shift (leading to the de-salienation of distinct, shift-inconsistent features on the train-time feature distribution).
This means that attackers should try to conform their data source to that of other attackers and the defender.
This also means that defenders should robustify their feature distributions against shift-inconsistencies; as stylization can also used as an augmentation procedure, we would expect data augmentation methods to be viable defenses as they should be able to discover these shift-inconsistencies, however this is not the case as shown in section \ref{3.5}. 

Second, we evaluate the shift combination of \{backdoor, adversarial\}.

\noindent\textbf{(Observation 2 cont'd)}
With respect to clean label accuracy, the introduction of adversarial perturbations push the accuracy down to 0.1 if it has not already been pushed down either by a backdoor attack or through the backfiring effect, as noted at $\varepsilon_{\textnormal{b}}, p = 0.2$ where the ASR was still larger than 0.1 before the adversarial attack. 

\noindent\textbf{(Observation 4: Interference between backdoor and adversarial perturbations)}
At $N=1$, we also note some interesting patterns in how adversarial perturbations sometimes contribute or hinder a backdoor attack in terms of poisoned label accuracy: 
specifically studying the range $\varepsilon_{\textnormal{b}}, p: 0.2, 0.4, 0.8$ across $\varepsilon_{\textnormal{a}}: 0.2, 0.4, 0.8, 1.0$, we find that at low $\varepsilon_{\textnormal{b}}, p$ an increasing $\varepsilon_{\textnormal{a}}$ contributes to and increases the backdoor ASR, but at high $\varepsilon_{\textnormal{b}}, p$ an increasing $\varepsilon_{\textnormal{a}}$ hinders and decreases the backdoor ASR.
There appears to be some form of interference taking place between the adversarial perturbations and backdoor perturbations: our hypothesis on this phenomenon is that when the poison rate is low against the surrogate model's gradients, FGSM is optimized towards pushing the inputs \textit{towards} the poisoned label, but when the poison rate is high then FGSM is optimized towards pushing inputs \textit{away} from the poisoned label. 
This appears to be counter-intuitive; from FGSM's point-of-view, the backdoor trigger presence should return perturbations that push the input's classification as far away from the poison label as possible (since from FGSM's viewpoint, the poison label is the ground-truth that it is trying to misclassify).
% {\color{blue} Explanation is in (https://openreview.net/pdf?id=8SP2-AiWttb), re-formualate it in my OWN proof as this is novel insight indeed w.r.t. backdoor attacks!
% Our explanation for this is as follows:
% it is acknowledged that a backdoor subnetwork (a subset of the gradients) would be very small (about 0.05\% of the parameter count) and that the real poison rate is very small (<0.01\%); hence, for any given input, even one with a backdoor trigger present, the gradients 
% while also bringing the poison label space closer the source label, hence easier to push across decision boundary
% My suspicion is that it has something to do with the proportion of the dataset being poisoned -- class imbalance, in the defender's dataset it is very different for 0.1 and 0.8 of dataset being the only 1 label

% Consider a one-dimensional classification task
% and a binary classifier with two outputs z1 and z2 (like logits
% of a DNN), Figure 1 illustrates the distributions of z1, z2 and
% z2 − z1 around x = 0. The classifier predicts class 1 when
% z1 ≥ z2, otherwise class 2. We consider an input at x = 0
% with correct prediction y = 1, and a maximum perturbation
% constraint  = 2 (e.g. perturbation δ ∈ [−2, +2]). The attack
% is successful if and only if z2 > z1. In this example, imbalanced gradients occurs at x = 0, where the gradients of the two
% terms ∇xz2 and ∇x(−z1) have opposite directions, and the
% attack is dominated by the z1 term as ∇x(−z1) is significantly
% larger than ∇xz2. Thus, attacking x with the margin loss will
% converge to +2, where the sample is still correctly classified.
% However, for a successful attack, x should be perturbed towards -2. In this particular scenario, the gradient ∇xz2 < 0
% alone can provide the most effective attack direction. Note that
% this toy example was motivated by the loss landscape of DNNs
% when imbalanced gradient occurs.

% }
With regards to $\varepsilon_{\textnormal{b}}, p = 1.0$ having such high ASR, it may not just be cause of a strong trigger pattern/saliency, but also it should be noted there is 100\% class imbalance in this case for the attacker's surrogate model (only 1 class in the training set, hence no decision boundaries to cross; adversarial ASR should be 0.0). 
Given that our intention for this experiment is to observe the effect of a joint distribution shift between these two attacks unmodified in procedure and aligned as much as possible to their original attack design, we did not construct a coordinated adversarial-backdoor attack where only adversarial perturbations that do not counter, or even reinforce, the backdoor perturbations / poison labels are crafted. 

Third, we evaluate the shift combination of \{adversarial, stylized\}.

\noindent\textbf{(Observation 5: Unaffected adversarial attack, if no trigger)}
Considering a poisoned dataset but a lack of backdoor trigger during run-time (i.e. run-time poison rate 0.0), we acknowledge that with the clean-label accuracy is stable for both stylization $\alpha$ attributed to the early-stopping training scheme. 
After adversarial attack (where both adversarial and stylized perturbations exist), we observe no significant differences between the tables between $\alpha=0.0$ and $\alpha=1.0$. This indicates that the generation of adversarial perturbations with respect to a contributed sub-dataset, even one with stylized shift from other sub-datasets, can still retain a high attack success rate even in a multi-agent backdoor attack. 
Additionally this gives the insight that an attacker can still pursue an adversarial attack strategy despite multiple agents; however, this may not necessarily always be practical, as the adversarial attack may not return a targeted misclassification of a specific target label (as evaluated in this experiment). 

Finally, we evaluate the shift combination of \{backdoor, adversarial, stylized\}.

\noindent\textbf{(Observation 4 cont'd)}
For low backdoor $\varepsilon_{\textnormal{b}}, p$, the adversarial $\varepsilon_{\textnormal{a}}$ contributes to increasing the accuracy w.r.t. poisoned labels, i.e. improving the attack success rate of the backdoor attack. This is consistent across stylization and number of attackers, except for $N=100, \alpha=1.0$.
However for higher values of $\varepsilon_{\textnormal{b}}, p$ at $N=1$, we note that after a certain threshold ($0.4$) of $\varepsilon_{\textnormal{a}}$, adversarial perturbations counter the backdoor attack for $\alpha=0.0$. For $\alpha=1.0, N=1$, $\varepsilon_{\textnormal{a}}$ continues to incrementally improve the backdoor attack.
For $N=100$, regardless of stylization, at high $\varepsilon_{\textnormal{b}}, p$, changes in $\varepsilon_{\textnormal{a}}$ do not significantly change the accuracy w.r.t. poisoned labels.
All of the 3 aforementioned patterns are identical and consistent with the patterns in \{backdoor, stylized\}, hence it leads us to believe that these changes are driven by stylistic perturbations rather than adversarial perturbations. 

\noindent\textbf{(Observation 2 cont'd)}
With respect to clean accuracy, we find that for low values of $\varepsilon_{\textnormal{b}}, p$, an increasing $\varepsilon_{\textnormal{a}}$ returns an improvement in attack success rate.
In general, we find that accuracy does not fall further than 0.1 (the lower bound in all our experiments).

% One of our suspicious regarding a low backdoor attack success rate is whether the generation of adversarial perturbations may possibly de-perturb backdoor perturbations: we visually inspect before-attack and after-attack images to verify that both adversarial and backdoor perturbations are retained in a multi-agent backdoor setting, and we sample a set in Figure \ref{} (Appendix \ref{}).
% We also find that training FGSM does not tend to undo the backdoor perturbation; we suspect the backdoor pattern is retained given ???
% Warning: The images are not correctly coloured, will this raise reviewer suspicions?
% (Mention that we leave this as a future work, if this is not figured out)

% Based on Third, can we argue about an alternative poison generated by FGSM?





% * Can we have 4 attack settings to evaluate in total? : 	
% 	1. Backdoor attack, where we maximize accuracy on poisoned labels
% 	2. (Poisoning?) attack, wehre we minimize accuracy on clean labels -- Warning: this would sort of be in contradiction to the goals of (1), no?
% 	3. Adv attack, where we maximize accuracy on own agent labels
% 	4. Stylized perturbations, where we maximize accuracy on own agent labels
% * Warning: Are we only using one variation of the adversarial attack algorithm? Are we using FGSM or PGD?	
% 	^ Based on tradeoff paper (https://papers.nips.cc/paper/2020/file/8b4066554730ddfaa0266346bdc1b202-Paper.pdf), we follow suite and use the PGD attack algorithm with l-inf constrain norm

% * Note on obj: the objective of an adversarial attack is very different from that of a backdoor attack -- for a successful adv attack, given a known dataset or trigger pattern being salient for an attacker's set, perturbing adversarially with respect to the trigger pattern should easily push ASR adv to 0.0, but in multi-agent, we would expect that the ASR does NOT go down to 0, as the trigger pattern saliency does not match between the 2 sets	

% Warning: Need to clarify on goal of adversarial attack case where attacker adds both eps_adv and backdoor_adv; in our current implementation, the defender (correctly) trains on a model based on backdoored triggers and clean labels, while attacker also generates via FGSM their samples with respect to backdoor triggers (is this bit correct, or should they generate with respect to clean labels?)	
% We demonstrate the first ever case of Adv Attack + Backdoor attack, and motivate it -- The multi-agent setting wipes out the ability for a backdoor trigger to work so it cannot trigger a targetted misclassification, but can it still attain an overall drop in robustness acc? We install backdoor trigger during test-time, and see if the conjoined effects of BOTH a backdoor pattern and adv pattern can pull down the clean acc, assuming they are not aiming for opposing labels	
% 	X -> T0
% 	X + eb -> T1 != T0
% 	X + ea -/> T0
% 	Hence, X + eb + ea -/> T0

% AdvTrojan (https://arxiv.org/pdf/2109.01275.pdf) combines both adv and backdoor perturbations to lower the ASR

% (https://arxiv.org/pdf/1703.06868.pdf) Page 8 shows how style varies with alpha, alpha=1 is not complete style image
% Perhaps we should show an example of joint shift input?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cooperation of agents}
\label{3.4}

In this section, we wish to leverage agent dynamics into the backdoor attack by investigating: can cooperation between agents successfully maximize the collective attack success rate?
% In this setting, we evaluate a different combination of actions by each individual attacker, and additionally evaluate their actions against a different combination of defender actions.
% Ideally, cooperation would be successful if they can return a robustly-high collective attack success rate across a range of defender actions.
The base case is $N=5$, $V_d = 0.1$, $p=0.55$, $\varepsilon=0.55$; the latter 2 parameters apply to the $N=100$ case; all 4 parameters apply to the Defense (Backdoor Adversarial Training w.r.t. Experiments \ref{3.5}) configurations) case.
We summarize the results for coordinated trigger generation in Table \ref{tab:coop2}, and the lack thereof in Table \ref{tab:coop1}.
% ; both tables contain results for every other strategy.
In addition, we record the escalation of poison rate and trigger label selection in Figure \ref{fig:escalation}. 

In this setting, we primarily study 2 variables of cooperation, which are also the set of actions that an attacker can take: (i) input poison parameters 
% (proportion of dataset to poison $p$, perturbation rate per input $\varepsilon$, distance between backdoor trigger patterns of different attackers)
($p, \varepsilon$, and distance between different attackers' backdoor trigger patterns)
, and (ii) target poison label selection. 
% We do not vary the action of backdoor attack algorithm, as backdoor attack algorithm variants follow the same principle but vary in trigger pattern and target label selection, which we account for here.
In addition to these 2 attacker actions that will formulate a set of strategies,
we wish to evaluate the robustness of these strategies by (i) testing the scalability of the strategy at very large attacker counts, and (ii) testing the robustness of the strategy by introducing the weakest single-agent backdoor defense. 
% 
% We would like to make some clarifications with respect to some terminology use.
% In traditional literature, the payoffs of each agent in a non-cooperative game would be the maximization of individual payoff, while that of a cooperative game would be that of collective payoff. 
% In a multi-turn game for DNN agents, agents could supposedly sample each other's distribution and adapt strategies; however, we establish a single-turn game (as a realistic and generalized backdoor attack assumes each attacker has no information of the other), and thus each agent only has their own distribution for reference.
% We raise the two topics of cooperation and turns, 
% because here 
We establish \textit{information sharing} as the procedure in which agents send information between each other, 
and the collective information garnered can return outcomes in the range of anti-cooperative (which we denote as agents using information that hinders the other agent's individual payoff) to cooperative (which we denote as agents using information to maximize collective payoff).
The payoff functions for anti-competitive and non-cooperative strategies (i.e. individual ASR) are the same.
% , we refer to them interchangeably. 
% We show the payoff for each individual attacker in our results to observe both effects.

% With these strategies, we would like to observe the following agent dynamics-driven phenomenon, specifically the outcomes from attackers exercising various extents of selfishness (escalating attack parameters) against extents of collective goodwill (coordinating attack parameters):
% (i) the outcome from the escalation of $\epsilon$; (ii) the outcome from a gradual coordination of target labels;, (iii) the outcome of coordinating trigger pattern generation.
% % \begin{enumerate}
% %     \item the outcome from the escalation of $\epsilon$;
% %     \item the outcome from a gradual coordination of target labels;
% %     \item the outcome of coordinating trigger pattern generation;
% %     % \item 
% % \end{enumerate}
% % From prior experiments, we are informed of the outcome of the escalation of poison rate (i.e. the collective attack success rate falls even further), hence we do not repeat this variable change in this setting.

% Variables of cooperation:	
% * Distance in trigger patterns : varies with poison rate, backdoor epsilon
% 	* Presence of defense
% * Number of attackers	
% * Selection of trigger/target labels	

% Here, we describe how we demonstrate selfish escalation or collective coordination.
% While in other experiments, we scale the effect of random selection to a large number of attackers to approximate non-cooperative behaviour, we would now like to simulate simplified cases of anti-cooperative and cooperative strategies. 
% For the selfish escalation of trigger patterns, we suppose each attacker crafts their backdoor trigger patterns independently from each other, and when information of the presence of other attackers is known or each attacker wishes to raise certainty of a backdoor attack, we consider the case where attackers to escalate their $\varepsilon$ from 0.15 to 0.55 to 0.95. 
% To study trigger label collision cases and coordinated target label selection, we show a gradual change in trigger label selection amongst attackers, where they start off each having independent labels, then there is some trigger label collision between 40\% of the attackers (40\% attackers sharing the same label), then there is 100\% trigger label collision between all of the attackers (i.e. all attackers share the same label). Coordination can manifest as either attackers each choosing distinctly different labels, or attackers all choosing the same label. To monitor collision between trigger patterns and trigger labels, we compute the cosine distance between each attacker's trigger pattern against that of Attacker Agent 1.
% The trigger patterns are randomly generated; first by computing a random set of pixel positional indices within image dimensions (pixel positions to be perturbed), which we refer to as \textit{shape} and show its corresponding cosine distance; then by computing the colour value change for each pixel position in the shape, which we refer this final trigger pattern of both positions and perturbations values as \textit{shape+colour}. We assume there is no coordination hence the choice of random perturbations (as opposed to a perturbation-optimization function of minimizing cosine distance), though as $\varepsilon$ increases, we note that the cosine distance for both shape and shape+colour decrease (as the density of perturbations would be expected to be higher as $\varepsilon$ increases); this provides us with a range of trigger pattern distances in the representation space to evaluate against trigger label selection.
% % Elaborate on trigger pattern coordination
% With regards to coordination of trigger patterns (as opposed to randomly-generated patterns), we again adapt our already-adapted implementation of \cite{gu2019badnets}, and introduce orthoginality between backdoor trigger patterns.
% Orthogonal trigger patterns should retain high cosine distances, and be far apart from each other in the representation space. 
% We optimize for maximizing cosine distance here for the reason that we suspect a possibility that the randomly-generated trigger patterns may in some cases incur feature collisions \citep{NEURIPS2019_7eea1f26}, where we have 2 very similar features but tending towards 2 very different labels; hence, it may be in the interest of attackers to completely minimize this occurrence and generate distinctly different trigger patterns that occupy different regions of the representation space. 
% We do not presume that this is a successful cooperation strategy; instead, we hold the definition of cooperation as very literal, in which a group of agents coordinate their values with respect to each others, rather than claiming a cooperative strategy is necessarily a strategy more successful than a non-cooperative one.
% One form of interepreting the intention of minimzing collisions between features (backdoor trigger patterns) is the intention of minimizing interference between these features; \citet{cheung2019superposition} introduced a method for continual learning where they would like to store a set of weights without inducing interference between them during training, and hence they generate a set of orthogonal context vectors that transforms the weights for each task such that each resulting matrix would reside in a very distant region of the representation space against each other.
% We adapt a similar implementation, but in the notion of applying an orthogonal matrix that transforms the backdoor trigger patterns into residing in a very distance region away from the other resultant trigger patterns.
% First, we generate a random trigger pattern using our multi-agent adaptation of \citet{gu2019badnets}, as used throughout the paper. 
% In-line with \citet{cheung2019superposition}, we sample orthogonal matrices from the Haar distribution, multiply it against the original generated trigger pattern (clip values for colour range [0, 255]) to return an orthogonal/distant trigger pattern.
% We show that the resulting trigger patterns tend to be distant from each other by including the cosine distance with respect to Agent 1, where a cosine distance of 1.0 indicates the 2 evaluated matrices are very distant from each other.
% % Elaborate on target label escalation or coordination

% # Rotational Superposition: They use scipy.stats.ortho_group to  to sample rotations uniformly from orthogonal group O(M) (Haar distribution)
% # Note: the matrices x being sampled are orthogonal given a seed value, meaning np.dot(x, x.T) would return an identity matrix; a set of matrices {x0, x1, ...} are not orthogonal to each other necessarily (?)
% # Sample an orthogonal matrix, multiply it with our base matrix, clip [0, 255], compute cos distance

% We evaluate on 5 classes: 0 (airplane), 2 (bird), 4 (deer), 6 (frog), 8 (ship); we retain the same proportions of each of these 5 classes as $N$ varies. 
% For $N=100$, we specify the number of attackers $N\{Y\}$ that target class $Y$.
% The base case is $N=5$, $V_d = 0.1$, $p=0.55$, $\varepsilon=0.55$, where all 4 parameters apply to the Defense (Backdoor Adversarial Training) case, and the latter 2 parameters apply to the $N=100$ case; other attack configurations are retained from Experiments \ref{3.1}.
% and all other backdoor defense configurations as Experiments \ref{3.5}.
% We retain a defender allocation of 0.1, poison rate $p$ of 0.55, specify labels and $\varepsilon$ and trigger pattern generation method, and retain all other attack configurations as Experiments \ref{3.1}.
% Except for the backdoor defense (in which the defense configurations for Backdoor Adversarial Training are identical to that in Experiments \ref{3.5}), 
% all other defense configurations are retained from Experiments \ref{3.1}.



% For the escalation figures, 
% we retain the aforementioned configurations with the following changes:
% in Table \ref{tab:coop1} and \ref{tab:coop2}, for agents without the escalation in overlap of target label 4 (in {\color{red}red}), we only redistribute the other 4 labels out equally, but in Figures \ref{fig:escalation} we redistribute 10 labels out randomly.
% We presume $N=100$.
% In the escalation plots, the mean and standard deviation should tend to be quite similar in aggregate across escalation, but what we are interested in studying is how the distribution itself changes, e.g. where do the quartiles/outliers lie.

\input{tables/cooperation}

% * We need scale up the epsilon and poison rate, as we have fewer attackers (ref to other tables where N=100 attackers usually needed)

% * Don't overdo this table; essentially it is just using orthogonal triggers, not "really" cooperation -- specify this section as just orthogonality tests I guess

% * Maybe stick to the proportion of the 5 setting, instead of using the whole trigger label range


\begin{figure}[]
    \centering
    \includegraphics[width=0.49\textwidth]{assets/escalation.pdf}
    \caption{(left) Coordination in terms of proportion of attackers selecting poison label 4, while others randomly select; (right) Escalation in terms of proportion of attackers increasing their poison rate from 0.15 to 0.55, while others retain 0.15, then subsequently the increase in poison rate from 0.55 to 0.95, while others retain their previously-escalated 0.55;  these escalation cases are plotted against corresponding distributions of poison label (top row) and clean label (bottom row) accuracies.}
    \label{fig:escalation}
\end{figure}

% Do a gradual escalation ablation study, to see how ASR decreases when trigger selection becomes more uniform, and when poison rate (NOT epsilon) gradually escalates
% Plot: % of agents picking 4 vs ASR
% Plot (a): % of agents switching from poison rate 0.15 to 0.55
% Plot (b): % of agents switching from poison rate 0.55 to 0.95

% Plot alt 1
% While on the topic of new plots, can we do a plot of t-SNE / feature space and compute the average distance along 2 weight axes as to how much a poisoned label has moved (distance) before and after the insertion of other agents? -- this would be very helpful
% https://github.com/spaceml-org/Interactive-TSNE
% Read up on how Goldstein ppl do it

% Plot alt 2
% What if we obtained the actual subnet responsible for the backdoor trigger, and tried to locate as number of attackers increase
% show a change in size (incl if the subnet does not exist at all), show change in distance (incl both mask shape as well as mask values)


% Minimum (Q0 or 0th percentile): the lowest data point in the data set excluding any outliers
% Maximum (Q4 or 100th percentile): the highest data point in the data set excluding any outliers
% Median (Q2 or 50th percentile): the middle value in the data set
% First quartile (Q1 or 25th percentile): also known as the lower quartile qn(0.25), it is the median of the lower half of the dataset.
% Third quartile (Q3 or 75th percentile): also known as the upper quartile qn(0.75), it is the median of the upper half of the dataset.[7]
% In addition to the minimum and maximum values used to construct a box-plot, another important element that can also be employed to obtain a box-plot is the interquartile range (IQR), as denoted below:

% Interquartile range (IQR) : the distance between the upper and lower quartiles
% {\displaystyle {\text{IQR}}=Q_{3}-Q_{1}=q_{n}(0.75)-q_{n}(0.25)}{\displaystyle {\text{IQR}}=Q_{3}-Q_{1}=q_{n}(0.75)-q_{n}(0.25)}

% \noindent\textbf{Findings. }
% We summarize the results for coordinated trigger generation in Table \ref{tab:coop2}, and the lack thereof in Table \ref{tab:coop1}.
% % ; both tables contain results for every other strategy.
% In addition, we record the escalation of poison rate and trigger label selection in Figure \ref{fig:escalation}. 

% Cases and outcomes:
% \begin{enumerate}
    % \item Escalation in poison rate (non-cooperative, anti-cooperative)
    % \item Gradual conformity in trigger selection (non-cooperative, cooperative)
    % \item Coordination of trigger pattern distance, both shape (very important, clash on same pixel positions) and colour (anti-cooperative, cooperative)
    % \item Changes w.r.t. Clean label acc
    % \item Changes w.r.t. N=100
    % \item Changes w.r.t. Defense
% \end{enumerate}

\noindent\textbf{(Observation 6: Futility of $p$-escalation)}
% First, we evaluate the set of anti-cooperative / non-cooperative strategies and their outcomes.
% Escalation in poison rate (non-cooperative, anti-cooperative)
In Figure \ref{fig:escalation} (right), 
we simulate an anti-cooperative strategy where attackers increasing escalate their poison rate in varying attacker count from 0.15 to 0.95. 
We find that the median poison label accuracy does not change significantly throughout, however small variations to the interquartile range take place, indicating that escalation of poison rate may not drastically change the overall outcome for attackers but it does indeed affect have an effect on the distribution of accuracy, i.e. the escalation of a group of attackers can certainly have an effect on the rest of the distribution of attackers.
Specifically, we find the interquartile range narrows when 80\% of the attackers all escalate, but that goes away once all attackers escalate to 100\% to 0.55: this is in-line with the expectation that once there is no discrepancy or steep gradient where most attackers have $p=0.55$ while only a few still have $p=0.15$, then the playing field for trigger pattern saliency is balanced once more.
We also observe a cyclical pattern in the max poison label accuracy and outliers (black scatter points above the boxplot), where it has tended to decrease when most agents have escalated, but tended to increase when few agents relatively escalated, and the resume at an average level when either no attackers or all attacekers have escalated.
Escalation is an intriguing aspect of this attack, as the attack success rate has as much to do with the order in which attackers coordinate (whether cooperatively or selfishly), as it does with the backdoor trigger pattern.

\noindent\textbf{(Observation 7: Futility of backdoor trigger pattern \& target poison label coordination)}
% Gradual conformity in trigger selection (non-cooperative, cooperative)
In Table \ref{tab:coop1}, one of the variations we study across all configurations is the outcome of attackers varying the overlap in target labels.
Trigger patterns are randomly generated, and the distance between them is strongly correlated with the perturbation rate $\varepsilon$, so we factor in this variance to show that this pattern is consistent and robust.
Regardless of $\varepsilon$ and trigger distance in shape or colour, or number of attackers; we find that if all $N$ attackers share the same trigger label, then a multi-agent backdoor attack can be successful.
There is a stark discrepancy in the range of values between each attacker picking different labels against all attackers picking the same label. 
Our initial hypothesis would have been that feature collision is the reason for this, however even when trigger patterns were distant from each other ($\varepsilon$=0.15), there is still a clear accuracy difference between identical vs non-identical target labels. We further investigate this feature collision hypothesis in Table \ref{tab:coop2} and Figure \ref{fig:escalation} (left).
What is more, the retainment of this high attack success rate is mutually beneficial (i.e. maximized collective ASR).
From an undefended multi-agent backdoor attack perspective, this would be considered a successful attack. However, one critical component of the payoff functions is that the attacker strategies also must be robust against defender strategies.
Unfortunately for the attackers, the worst-performing single-agent backdoor defense (according to Experiments \ref{3.5}) cuts the attack success rate by a large margin; the collective ASR may not be as low as other trigger overlap settings under this defense, but it still is significantly lower than No Defense cases.
{\color{blue} To further support this conjecture and why not to underestimate the importance of defender strategies in determining success of an attack, 
the definition and computation of the Nash equilibrium dictates that an agent's strategy is the equilibrium if the strategy payoff value cannot be further increased given the entire range of opponent strategies. 
In this case, the dominant strategy of the defender is to enforce a backdoor defense, and no attack configuration is demonstrated where the mean payoff of this strategy would be lower than to not enforce a defense: this means we need to evaluate configurations with respect to a defender picking this strategy, and the equilibrium case where attacker(s) can maximize their payoff(s) is if they coordinate their trigger label selection, resulting in a mean (attackers, defender) equilibrium payoff of (25.4, 74.6)\%.
}
Hence, we would argue that coordinating constant labels amongst attackers is not a robust strategy.
In addition, we show the converse, that escalation of trigger patterns to be non-identical and personalized to each attacker's respective sub-datasets acts against individual and collective ASR. In practical settings, not only will sub-datasets encounter sub-population shift or domain shift, they may also have heteregeneous class/sub-class sets (i.e. attackers may wish to poison labels that are very specific to them, but not contained in other attacker's sets). 
For example, in a dataset containing a class 'dogs', there may be numerous sub-classes of dogs; so even though a set of attackers share the same class set, if they share different sub-class sets and each attempt to poison a target label that is contained in other attacker sub-datasets but is not selected for poisoning, then they are hindering themselves as well as other attacker ASRs (and we also remind that it is indicated thus far that the trigger label selection has a greater impact than the trigger pattern and features, so even if an attacker poisons a very niche sub-class, if the poisoned input is assigned a common/shared class, which may be the case if it is human-labeled by defender, then the backfiring effect will still manifest). 

While on the topic of trigger pattern overlap, none of these patterns manifest when trigger patterns are orthogonal to each other (Table \ref{tab:coop2}).
Regardless of $\varepsilon$ changes, orthogonally-coordinated trigger patterns do not sustain comparatively high ASR as that generated randomly, regardless of poison label overlap.
{\color{blue} What is puzzling is that the cosine distance is comparatively high as that when the poison rate is low. 
What could cause this? Is it something to do with orthonormal and centroid distances?
If we refer to the insight on orthogonal gradient descent (https://arxiv.org/pdf/2106.15023.pdf), they show that the interference between 2 distant inputs can be resolved by computing orthogonal losses. This would be in-line with both the super-position paper and our results w.r.t. clean labels accuracy, if we can show that orthogonal triggers (w.r.t. Eqt3 on loss) results in orthogonal loss components that inadvertently results in orthogonal gradient descent.
}
Our hypothesis is that the target label overlap has a significant benefiting effect on collective ASR only when the trigger patterns are close to each other in the feature space (i.e. when cosine distance is low). This is the consistent pattern thus far.
In general, we observe that the collective attack success rate is inversely proportional to the cosine distance of trigger patterns between attackers.

In addition, we wished to observe whether there is any benefit to attackers cooperating in sub-groups to coordinate trigger label selection. In both Tables, we find that when 40\% of attackers choose the same target label, there is no clear unilateral increase in their individual ASR compared to the other attackers; in fact, some other attackers may even have higher individual ASR. 
Though a gradual shift towards overlapping target poison labels did not yield a clear pattern when $N=5$, in the $N=100$ case there is a clearer proportionality where when the number of attackers is very large, when the sub-group of attackers coordinating their target labels increase, the collective ASR tends to increase.
We also attribute this phenomenon in $N=5$ to the notion that the proportion of trigger label overlap had not reached a critical threshold, and non-cooperating attackers happened to have trigger patterns more salient for their target label than even cooperating ones.
We demonstrate this threshold effect in Figure \ref{fig:escalation} (left), where if the proportion of attackers coordinating their labels is less than 80\%, then the distribution of individual ASRs are extremely wide; there is some indication that some attackers may be able to enjoy high ASR given the consistently increasing max and upper-quartile values as the proportion of overlapping participants increase, but as shown in Table \ref{tab:coop1} this does not guarantee that the participating colluders will necessarily reap this benefit.
Hence it generalizes a pattern of equity: the only times the collective ASR drops is when there is gross inequity between attackers (where some attackers have not escalated yet); when all attackers escalate again, the distribution of ASR resumes back to a comparable level.



% \item Coordination of trigger pattern distance, both shape (very important, clash on same pixel positions) and colour (anti-cooperative, cooperative)
Now we would like to consider cooperation with respect to trigger pattern generation. Though the random trigger pattern adaptation of BadNet renders unique patterns, it is clear from Table \ref{tab:coop1} that the resulting distance between the patterns varies on many factors such as perturbation rate. 
Based on the notion of interference minimization (as the loss function we discussed in section \ref{} aligns with the transfer-interference tradeoff cited in \cite{}), we would like each attacker to generate trigger patterns that do not interfere with each other (i.e. orthogonal to each other, and reside in distinctly separate and distance subspaces from each other in the input space) regardless of factors such as perturbation rate. 
This is enabled from information sharing.
As mentioned before, we do not conclude this to be a cooperative attack based on an assumption that the attack will be successful (so do not hold it against the results that they are invalid simply because the attack failed), we presume it as such because of information sharing, motivated by equations \ref{}.
The results indicate that information sharing with respect to trigger pattern orthogonality still does not yield favourable collective ASR. 
We verify that the shape distance is large (i.e. the positional indices of each perturbed pixel is also distinctly distant) as well as the colour+shape distance.
However, in all such cases, the collective ASR stays low, even when there is 100\% trigger label overlap. 
Consequently, this supports the empirical evidence and theoretical reasoning thus far that the true issue is not a feature collision between trigger patterns, else this attack would have been successful.
While this is just one of a few information sharing strategies evaluated (the other being on target trigger label), these results do not conclude that there does not exist an information sharing strategy that can unilaterally cause a successful multi-agent backdoor attack; instead, we introduce information sharing variants to evaluate the introduction of the attack, as well as the feature collision hypothesis.

% \item Changes w.r.t. N=100


% \item Changes w.r.t. Defense


The final (but not tabulated separately) form of information sharing resulting in a cooperative attack is one where attackers coordinate such that they all have 1 identical trigger patter, and 1 identical target poison label, i.e. they collectively approximate a single-agent attack. The ASR is approximately that of a single-agent backdoor attack. Other than the downside of not being able to flexibly curate the attack to their needs (e.g. targeted misclassification), single-agent backdoor attacks have been shown in literature as well as Experiments \ref{3.5} to be mitigatable, hence this extreme extent of information sharing also does not yield a successful attack.
In fact, an extension of this is shown in Table \ref{tab:coop1}, where we have a set of low-distance trigger patterns, inadvertently due to a high $\varepsilon$.
It shows that if a set of attackers were to coordinate such they minimized the cosine distance between their trigger patterns, (i) if each attacker were to pick distinctly different target labels, the successful individual ASR would be random (as indicated where 1 attacker had a successful ASR while the others reached ASR=0.0), and (ii) if all attackers picked the same label, then even though the trigger pattern is not identical, the ASR for these agents would still be collectively high.
This is in-line with results from \cite{9211729}, where the authors 
implemented 2 single-agent backdoor attacks with multiple trigger patterns with expectedly low distance from each other (one attack where the trigger patterns are of varying intensity of one pattern; another attack where they compose different sub-patterns, and thus different combinations of these sub-patterns would compose different triggers of low-distance to each other), and demonstrated that the attack success rate can be retained to be high, in addition to being more resilient against backdoor defenses.
Intuitively, our result for low-distance trigger patterns with same shared labels make sense, as there is no collision in features. The trigger pattern features overlap means there is a trigger sub-region (or overlapping region between trigger patterns) that becomes even \textit{more} salient and is reinforced during training (a robust backdoor trigger pattern/sub-pattern).
One could have argued that an optimal multi-agent backdoor strategy would be minimize cosine distance, where if attackers generate patterns of low orthogonality, then the trigger label cooperation case can maximize their collective ASR.
However, a cooperative attack with non-orthogonal triggers but same label can reduce their ASR to 0 with the inclusion of a backdoor defense due to it approximating a single-agent backdoor attack, regardless of a robust trigger sub-region. This cooperative setting may even be the weakest setting, weak because it requires attackers to share information that can be used against them (e.g. anti-cooperative behaviour such as escalation), and weak because of how easily it can be defended against.
% * Warning: At HIGH poison rates, the similarity of trigger patterns is extremely high due to large size of the trigger pattern	

\noindent\textbf{(Observation 2 cont'd)}
% \item Changes w.r.t. Clean label acc
Consistent with all prior results, the clean label accuracy tails off at 0.1. 
We note that the accuracy is higher when the $\varepsilon$ is lower in Table \ref{tab:coop1}, but more importantly we note that the clean label accuracy is significantly higher across all settings in Table \ref{tab:coop2} with orthogonal triggers than without. 
Orthogonal backdoor triggers \citep{} are demonstrated in existing literature to work, as regardless the distance from other trigger patterns, the principles of a backdoor attack are still upheld where static patterns of pixels on a set of poisoned inputs are passed into a training model to learn these patterns to be salient. 
{\color{blue} Why is this the case? What is our explanation?}
% 	Oddly enough, the Run-time acc wrt clean labels approximates the Validation acc !!!
{\color{red}
The acc w.r.t. poisoned labels and acc w.r.t. clean labels are all near 0.1.
While we could have argued that this is due to clean labels equalling poison labels, 
the more likely phenomenon is that when a backdoor trigger is present, the model engages in random guessing the label. In experiments \ref{3.2}, it is clear that the model can predict accurately on clean inputs, so it the model has not degraded completely, it just selectively degrades with respect to backdoored inputs.
}


% Second, we evaluate the set of cooperative strategies and their outcomes.

% ^Q: why when 2 labels are the same, but one has ASR 9x while the other has ASR 0? Shouldn't both be 9x?
% We include the 2 4s case, not for escalation reasons (else reviewer asks why no escalation for poison rate), but to see is there a middle ground, like with alpha
% First we conclude that same-trigger can still retain collective ASR, but when would it get further reduced? Introduce use of subset removal (defender actions), scale up number of attackers (capacity), increase poison/epsilon of other attackers (attacker MAD)
% * Why can everyone retain high ASR when same trigger? What kind of escalation would need to occur for same-trigger setting to suffer in ASR loss? Why would the use of different triggers have such a big difference from using same trigger w.r.t. capacity?
% * For all the other experiments, we use random trigger label selection -- when the labels coincide, then those attackers can maximize their ASR
% * Alternatively, I can just set the eps=0.95, then the trigger issue won't occur
% We argue that even the weakest multi-agent backdoor defense can mitigate this circumstance
% Intuitively, low distance trigger patterns with same labels make sense, as there is no collision in features, trigger feature overlap means there is a trigger sub-region that becomes even more salient and is reinforced during training (robust backdoor trigger pattern!)

% ASR is definitely correlated with orthogonality (when trigger label constant)	
% * Warning: the use of orthogonal triggers also increasing clean accuracy is quite concerning…or is it? It is a good thing, no?	
% 	Supposedly if the ASR goes down, it means the defender's clean accuracy is up?
% Maybe we leave out the Defender Validation Acc?	
% 	Oddly enough, the Run-time acc wrt clean labels approximates the Validation acc !!! -- this is an impressive value! -- very important, orthoginality has large impact on clean label accuracy of poisoned inputs
% 	* So the inference we make here, is that for the same trigger algorithm, if attackers generate patterns of low orthogonality, then trigger label cooperation can maximize their collective ASR
% * However, using cooperative attack with low orthogonal triggers but same label can reduce their ASR to 0 with the inclusion of a backdoor defense -- hence this cooperative setting is actually the weakest setting	
% 	* it requires cooperation, hence is the weakest setting
% 	* it can be wiped out by defenses, hence is the weakest setting
% * Warning: At HIGH poison rates, the similarity of trigger patterns is extremely high due to large size of the trigger pattern	
% 	* Hence, we need to use a low poison rate setting as ablation

% In terms of escalation, the pattern we observe is one of equity: the only times the collective ASR drops is when there is gross inequity between attackers (where not attackers escalated yet); when all attackers escalate again, the distribution resumes back to normal -- pay attention to upper quartile and outliers
% Based on the 2 Tables, we wish to evaluate 2 types of escalations: (i) where they share more target labels, or (ii) they increase their poison rate


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Performance against Defenses}
\label{3.5}

In this section we wish to investigate: how do the use of single-agent backdoor defenses affect the outcomes of the multi-agent backdoor attack?
% The use of a defense is an important component of this one-turn game, as the choice of a defense may not be known to any attackers, and in order for attackers to maximize payoff, they would need the multi-agent attack to retain a high individual and collective attack success rate against any defender model configuration. 
$V_d = 0.8$, $\varepsilon, p = 0.55$, 
% run-time poison rate is $1.0$, 
and target poison label for each attacker is randomly selected. 
Defenses are evaluated on the Clean Label Backdoor Attack \citep{turner2019cleanlabel} in addition to BadNet.
Results are summarized in Figure \ref{fig:defenses}. 
Specifically, we evaluate 2 augmentative and 2 removal defenses:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item \textit{No Defense: }
    We retain identical defender model training conditions to that in Experiments \ref{3.1}. 
    % An additional defense would be added on top of this baseline configuration. 
    The defender allocation $0.8$ would be unmodified during model training in this setting.
    % explanation of defense
    % config of defense
    
    \item \textit{Data Augmentation: }
    Recent evidence suggests that using strong data augmentation techniques~\citep{9414862} 
    % (e.g.,  CutMix~\citep{Yun_2019_ICCV} or MixUp \citep{zhang2018mixup}) 
    leads to a reduced backdoor attack success rate.
    We implement CutMix~\citep{Yun_2019_ICCV}, where augmentation takes place per batch, and training completes in accordance with aforementioned early stopping.
    % where $50\%$ of the defender's allocation of the dataset is assigned to data augmentation (i.e. for $V_d = 0.8$, 0.1 clean fracs, 0.1 augmented with CutMix
    
    \item \textit{Backdoor Adversarial Training: }
    \citet{geiping2021doesnt} extend the concept of adversarial training %(i.e., including an adversarial loss in the objective) 
    on defender-generated backdoor examples to insert their own triggers to existing labels.
    % ; this leads to a reduction in saliency of existing attacker triggers.
    % Rather than using an adversarial loss as in~\citep{geiping2021doesnt}, 
    % We augment the training data with defender-generated backdoor examples directly. %, to supplement one of our hypotheses pertaining to agent augmentation.
    We implement backdoor adversarial training~\citep{geiping2021doesnt}, where the generation of backdoor perturbations is through BadNet~\citep{gu2019badnets}), 
    where $50\%$ of the defender's allocation of the dataset is assigned to backdoor perturbation (i.e. for $V_d = 0.8$, $0.5 \times 0.8$ is clean while $(1-0.5) \times 0.8$ is perturbed),
    where $p, \varepsilon = 0.4$, 
    % poison rate and backdoor epsilon are $0.4$, 
    and where there are 20 different backdoor triggers used (i.e. allocation of defender's dataset for each backdoor trigger pattern is 
    $0.5 \times 0.8 \times \frac{1}{20}$
    % $0.5*0.8*0.05$
    ). 

    \item \textit{Spectral Signatures: }
    Spectral Signatures~\citep{NEURIPS2018_280cf18b} is an input inspection method used to perform subset removal from a training dataset. 
    % For each class in the backdoored dataset, the method uses the singular value decomposition of the covariance matix of the learned representation for each input in a class in order to compute an outlier score, and remove the top scores before re-training.
    In-line with existing implementations, we remove the top 5 scores for $N=1$ attackers. For $N=100$, we scale this value accordingly and remove the top 500 scores.
    % 'num_samples_to_remove' : 480, # Spectral_Signatures
    % * Spectral signatures, remove 5 items -- N=1
    % * Spectral signatures, remove N=480 items for N=100 ; set N=0.008*60000=480 as worst-case -> some triggers get pruned out, making it easier for other attackers!
    % https://proceedings.neurips.cc/paper/2018/file/280cf18baf4311c92aa5a042336587d3-Paper.pdf
    
    \item \textit{Activation Clustering: }
    Activation Clustering~\citep{chen2018detecting} is also an input inspection method used to perform subset removal from a training dataset. 
    In-line with \citet{chen2018detecting}'s implementation, we perform dimensionality reduction using Independent Component Analysis (ICA) on the dataset activations, then use \textit{k}-means clustering to separate the activations into two clusters, then use Exclusionary Reclassification to score and assess whether a given cluster corresponds to backdoored data and remove it.
    % 'nb_dims' : 10, # Activation_Clustering
    % https://arxiv.org/pdf/1811.03728.pdf
    
\end{itemize}



\input{tables/defenses}

% * Note: there are no issues with our implementation, it is correct that the accuracy with respect to poisoned labels for N=1 goes from 0.9x to 0.x!!!
% * What is more concerning (and probably best to leave out) is that the clean label accuracy still stays low
% * Clean-label activ clustering & backdooradvtraining did not work; poisoned label & clean-label acc is identical (0.553); or maybe for clean-label attack, this is expected!
% * If we can show no-defense ASR of over 9x%, then a 0.7x data augmentation performance is actually in-line! (https://arxiv.org/pdf/2011.09527.pdf)
% * Warning: numbers not making sense is a legitimate reviewer argument
% * Would be better to just leave out badnet with the simple implementation; just give technical explanation

% * To the contrary, we find that data augmentation worsens the mult-agent collective ASR (though we confirm it can reduce for single attacker, which would be in-line with citation?!)
% * Spectral signatures, may be interesting to see results on varying N removed items
% * In a multi-agent setting, ASR is already pretty bad, we're just showing that defenses actually make things worse
% * Need to show that Clean-Label Attack also returns low ASR

% Attacker configurations:
% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    % \item 
% $V_d = 0.8$, $\varepsilon, p = 0.55$, 
% % run-time poison rate is $1.0$, 
% and target poison label for each attacker is randomly selected. 
% All other attack configurations are identical to that in Experiments \ref{3.1}.


    % \item 
% In addition to BadNet, we also evaluate defenses on the Clean Label Backdoor Attack \citep{turner2019cleanlabel}.
% Also a common baseline backdoor attack algorithm, 
% the main idea of their method is to perturb the poisoned samples such that the learning of salient characteristic of the input more difficult, hence causing the model to rely more heavily on the backdoor pattern in order to successfully perform label classification. It utilizes adversarial examples or GAN-generated data, such that the resulting poisoned inputs appear to be consistent with the clean labels and thus seem benign even upon human inspection.
% The objective of a targeted clean label poisoning attack \citep{10.5555/3327345.3327509} (which also applies to a clean label backdoor attack), is to introduce backdoor perturbations to a set of inputs during train-time whose poisoned labels are equal to their original clean labels, but the usage of the backdoor pattern during run-time regardless of ground-truth class would return the poisoned label.
% We align our implementation with that of \citet{turner2019cleanlabel}, and use projected gradient descent (PGD) \citep{madry2018towards} to insert backdoor perturbations $\varepsilon$. 
% % \end{itemize}
% 
% Defense configurations:

% \noindent\textbf{Findings. }
\noindent\textbf{(Observation 2 cont'd)}
In this case, a lower accuracy w.r.t. poisoned labels infers a better defense. While a post-defense accuracy below 0.1 is indicative of mislabelling poisoned samples whose ground-truth clean labels were also poisoned labels, it is also at least indicative of de-salienating the backdoor trigger perturbation, and hence indicative of backdoor robustness.

For $N=1$, we observe strong defense performance against BadNet and reasonable defense performance against Clean-label Backdoor attacks, in-line with reported values in literature. 
This is in strong contrast to the defense performance at $N=100$. 
For the Clean-label backdoor attack, though the attack success rate is lower across all defenses at $N=100$ than no defense at $N=1$, we acknowledge this drop in ASR is likely to be attributed to both the defense itself as well as the backfiring effect to varying extents. The subset removal methods have strong reduction in ASR against clean-label attacks compared to the No Defense ASR so it could be argued that the defenses are sufficiently strong; however, the ASR even increases for the augmentation strategies, countering the backfiring effect and improving collective ASR. 
Considering BadNet, the ASR across diffenses are similar to the No Defense ASR in value, and the $\texttt{mean + std}$ value even increases in ASR for almost all defenses except activation clustering. 
% The results from this experiments are cautionary in nature: it indicates that existing single-agent backdoor defenses may not be prepared to robustify models against multi-agent backdoor attacks (which we motivate to be a practical setting), and may in contradiction even worsen the ASR. 


% If we can show no-defense ASR of over 9x\%, then a 0.7x data augmentation performance is actually in-line! (https://arxiv.org/pdf/2011.09527.pdf)

% To the contrary, we find that data augmentation worsens the mult-agent collective ASR (though we confirm it can reduce for single attacker, which would be in-line with citation?!)

% Spectral signatures, may be interesting to see results on varying N removed items

% In a multi-agent setting, ASR is already pretty bad, we're just showing that defenses actually make things worse

% Need to show that Clean-Label Attack also returns low ASR


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Recommendations}


% % Insights:
% 1. May not need explicit defenses; multi-agent attackers are in itself a natural defense, the use of defenses may hinder us inadvertently, both increasing ASR while reducing standard accuracy -- if defender accounts for all dynamics, incl poison rate, existing defenses, cooperation, escalation, etc, then there is action that attackers can take that can unilaterally increase their ASR w.r.t other attackers and retain high ASR against defender
% 2. Increasing the complexity in input/feature distributions (e.g. incr complexity of train-time dist with multiple triggers, stylistic changes; incr in complexity of test-time dist with adv layered on backdoor trigger) makes it difficult to use defenses used for single robustness use case -- distribution management is an important concern, with 1 trigger it creates saliency, but with multiple triggers the distribution and salient features are smoothened/avereged out (de-saliency effect that causes backfiring effect), but with the use of additive/reductive defenses we change change saliency of features in distribution again -- Hendrycks showed that diff adaptation strategies are worse off than simple large MLPs due to capacity reasons, perhaps it is not just capacity, but also because these different methods bring tradeoffs or harmful shifts to the distribution?
% 3. 


% IMPORTANT: Critical consideration of baselines
% For defenses, we motivate a new baseline; natural defense setting (no interventionm N=100), the baseline should not just be "no defense, N=1".
% For attacks, we motivate a new baseline for showing attack success; instead of just optimizing attacks against defenses, we should consider optimizing attacks against this backfiring effect; even with no defenses, all these top-tier attacks fail, and even need the help of defenses to work.

==> 4b.findings.tex <==
% \subsection{Findings}
% \noindent\textbf{Findings}
\subsection{Findings}

The main takeaway from our findings is the phenomenon, denoted as the \textit{backfiring effect},
where a backdoor trigger pattern
will trigger random label prediction
and attain lower-bounded collective attack success rate.
It demonstrates the following properties:
\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item 
    \textit{(Observation 1)} 
    Backdoor trigger patterns tend to return random label predictions, and thus
    the collective attack success rate converges to the lower bound. 
    \item 
    \textit{(Observation 2)}
    Observation 1 is resilient against most combinations of agent strategies, 
    particularly variations in defense, and cooperative/anti-cooperative behavior.
    \item 
    \textit{(Observation 3)}
    Adversarial perturbations are persistent and can co-exist in backdoor-perturbed test-time inputs while successfully lowering accuracy w.r.t. clean labels (Appendix \ref{aEF}).
    \item 
    \textit{(Observation 4)}
    Model parameters at $N>1$ become distant compared to $N=1$, but for varying $N>1$ tend to be similar to each other (Appendix \ref{aEF}).
\end{enumerate}

% \noindent\textbf{(Observation 1: Backfiring effect)}
% A phenomenon, denoted the \textit{backfiring effect}, occurs
% where the backdoor trigger patterns of multiple backdoor attackers
% will trigger random label prediction
% and attain lower-bounded collective attack success rate.
% We provide further explanations in Section \ref{}.

\noindent\textbf{(Observation 1: Backdoor-induced randomness)}
Across \mybox{(E1-6)}, as $N$ increases, the collective attack success rate decreases.
In the presence of a backdoor trigger pattern, the accuracy w.r.t. poisoned and clean labels converge towards the lower-bound attack success rate (0.1).
In \mybox{(E1)}, across $N$, at each $\varepsilon$ the standard deviation is similar; but as $\varepsilon$ increases at each $p$, the standard deviation also increases, i.e. anti-correlation between the mean and standard deviation.
% 
Varying across datasets \mybox{(E2)}, the drop in the accuracy w.r.t. defender's validation set (containing clean labels of unpoisoned inputs and poisoned labels of poisoned labels) between $N=1$ to $N=100$ is close to negligible (with slight drop for STL10).
Most attacker's poison allocation is allocated to run-time than train-time, hence the real poison rate is small, and the defender validation accuracy faced minimal impact with respect to the reduction in accuracy w.r.t. poisoned labels. 
% 
In \mybox{(E3:  \{backdoor, adversarial\})} and \mybox{(E3: \{backdoor, adversarial, stylized\})},
we find that the introduction of adversarial perturbations pushes the accuracy w.r.t. clean labels down to 0.1 if it had not already reached this lower bound through the backfiring effect. 
We observe this at low values of $\varepsilon_{\textnormal{b}}, p$ (e.g. $\varepsilon_{\textnormal{b}}, p = 0.2$), where \textit{ASR>0.1}
before the adversarial attack,
and 
observe the discrepancy between backfiring and adversarial attack comparing $\varepsilon_{\textnormal{b}}, p = 0.0$ against $\varepsilon_{\textnormal{b}}, p > 0.0$.


\mybox{(E2)}
In-line with \citet{10.1145/3474085.3475591} and our results for $N=1$, 
% we learn that a single-agent backdoor attack is capacity-agnostic, 
we validate that even large capacity models can be backdoored. 
At $N=1$, there is a general inverse pattern where the larger the model capacity, the lower the accuracy w.r.t. poisoned labels. 
% This is in-line with \cite{}, where we would expect a larger poison rate would be needed to render a subnetwork in a larger capacity model. 
Our expectation would be that for larger capacity models, they would be able to retain more backdoor subnetworks of multiple agents. However this is not the case: even as small as 5 attackers, we find that the mean accuracy for all models has already fallen to below 0.4, and there is a consistent decline for both the mean and standard deviation, where the values are similar across all models at each $N$; i.e. backfiring is independent of model capacity. 

\mybox{(E3: \{backdoor, stylized\})} 
For run-time poison rate 0.0 (poisoned at train-time, but not run-time), 
% one interesting phenomenon we  would like to point out is that 
the accuracy w.r.t. clean labels is low \textit{only when the backdoor trigger is present}; when the backdoor trigger is \textit{not} present, be it $N=1,100$ or $\alpha=0.0, 1.0$, a high clean label accuracy is retained, as high as a model trained on a dataset with no backdoor attack at all. 
% This is important to note, as 
This means the multi-agent backdoor attack does \textit{not} violate the secondary objective of the attacker, which is that the backdoor attack does not affect standard performance on clean inputs. 


\mybox{(E3: \{backdoor, stylized\})} 
For run-time poison rate 1.0, 
at $N=1$ the stylized perturbations do not affect the accuracy w.r.t. poisoned labels.
At $N=100$, stylized perturbations contribute to further decrease in accuracy w.r.t. poisoned labels, particularly at high $\varepsilon_{\textnormal{b}}, p$. 
Intuitively, we would expect that the stylization would strengthen a backdoor trigger pattern, in-line with literature where backdoor triggers are piece-wise \citep{9211729}.
Theorem 1 supports this sustained backfiring effect despite stylization, as the distribution of $\varepsilon \mapsto y_{i}$ would still tend to be random.
It suggests that trigger strengthening (or joint saliency) would be unlikely to manifest, even if stylization is applied to poisoned inputs only.
The additional texture shift to some extent contributes to backfiring, meaning attackers should try to conform their data source to that of other attackers and the defender. This also means that defenders should robustify the joint dataset against shift-inconsistencies; as stylization can also used as an augmentation procedure, we would expect data augmentation methods to be viable defenses as they should be able to discover these shift-inconsistencies, though this is not the case in E5.

\mybox{(E4)}
We note that the accuracy w.r.t. clean labels is higher when the $\varepsilon$ is lower in Table \ref{tab:coop1}, and observe that the accuracy w.r.t. clean labels is significantly higher across all settings in Table \ref{tab:coop2} with orthogonal triggers than without. 
Orthogonal backdoor trigger patterns, alike to randomly-generated trigger patterns, retain the same principles of a backdoor attack, where static patterns of pixels on a set of poisoned inputs are passed into a training model. 
% {\color{blue} Why is this the case? What is our explanation?}
% 	Oddly enough, the Run-time acc wrt clean labels approximates the Validation acc !!!
% {\color{red}
% The acc w.r.t. poisoned labels and acc w.r.t. clean labels are all near 0.1.
% While we could have argued that this is due to clean labels equalling poison labels, 
% the more likely phenomenon is that when a backdoor trigger is present, the model engages in random guessing the label. 
% In experiments \ref{3.2}, it is clear that the model can predict accurately on clean inputs, so it the model has not degraded completely, it just selectively degrades with respect to backdoored inputs.
% }

\mybox{(E5)}
For $N=1$, we observe strong defense performance against BadNet and reasonable defense performance against Clean-label Backdoor attacks, in-line with reported values in literature. 
This is in strong contrast to the defense performance at $N=100$. 
For the clean-label backdoor attack, though the accuracy w.r.t. poisoned labels is lower across all defenses at $N=100$ than no defense at $N=1$, this drop can be attributed to both the defense as well as the backfiring effect. The subset removal methods have strong reduction in ASR against clean-label attacks compared to the \textit{No Defense} ASR so it could be argued that the defenses are sufficiently strong; however, the ASR even increases for the augmentation strategies, countering the backfiring effect and improving collective ASR. 
Considering BadNet, the ASR across defenses are similar to the \textit{No Defense} ASR, and the $\texttt{mean + std}$ value even increases in ASR for almost all defenses except activation clustering. 
% may remove this next sentence:
The results from this experiments are cautionary in nature: it indicates that existing single-agent backdoor defenses may not be prepared to robustify models against multi-agent backdoor attacks (which we motivate to be a practical setting), and may in contradiction even worsen the ASR. 

Theorem 1 aids in explaining that the presence of a backdoor trigger pattern during run-time will induce a random label prediction, and as the attack parameters escalate, the likelihood that the collective attack success rate will tend towards the lower bound (0.1). 
It shows that the accuracy w.r.t. clean labels can be retained for clean inputs (i.e. no backdoor trigger pattern). 
% Why do adv perturbations push to 0.1? This is unclear
% Why do the defenses rebounce ASR back to 0.1?
Though backdoor defenses can reduce the ASR between \textit{No-Defense} to \textit{With-Defense} for $N=1$,
it has not been able to replicate this same drop in $N>1$, 
indicating that existing augmentative and removal defenses may not sufficiently mitigate the tendency for $f(\varepsilon; \theta) \sim \texttt{Rand}$.

With respect to stylized perturbation,
a well-trained model may have learnt to isolate $\mathbf{x}$ from $\varepsilon_{\textnormal{noise=style}}$ to return correct classifications.
With respect to adversarial perturbation,
$\varepsilon_{\textnormal{noise=adversarial}}$ does not have the $\varepsilon$-interference issues of backdoor triggers patterns (i.e. no consideration of $\varepsilon_{\textnormal{noise=adversarial}}$ of different attackers required, given in our setup they all use the same source dataset), hence are not hindered in adversarial attack success rate.


% \noindent\textbf{(Observation 1b: Change in trigger saliency)}

% \noindent\textbf{(Observation 3: Low accuracy w.r.t. clean labels with trigger)}
% (E2) One visible downside of the multi-agent backdoor attack presented here, and consistent with experiment results in other sections, is the low clean label accuracy when poison rate = 1.0. Though the backdoor attack's primary objective has failed for the attackers (maximizing accuracy w.r.t. poisoned labels), the attackers successfully poison the model into make faulty predictions, and even the use of backdoor defenses cannot retain clean label accuracy.









\noindent\textbf{(Observation 2: Futility of optimizing against $a_{\neg i}$/$d$ strategies)}
% \noindent\textbf{(Observation 2: Futility of strategy)}
% \noindent\textbf{(Observation 6: Futility of $p$-escalation)}
% First, we evaluate the set of anti-cooperative / non-cooperative strategies and their outcomes.
% Escalation in poison rate (non-cooperative, anti-cooperative)
\mybox{(E4)}
In Figure \ref{fig:escalation} (right), 
we simulate an anti-cooperative strategy where attackers increasingly escalate their poison rate in varying participating attacker proportion from $p=0.15 \rightarrow 0.95$. 
% We find that the median poison label accuracy does not change significantly throughout, however small variations to the interquartile range take place, indicating that escalation of poison rate may not drastically change the overall outcome for attackers but it does indeed affect have an effect on the distribution of accuracy, i.e. the escalation of a group of attackers can certainly have an effect on the rest of the distribution of attackers.
We find that the median accuracy w.r.t. poisoned labels does not change significantly, however small variations to the interquartile range take place, indicating that escalation of poison rate may not drastically change the overall collective attack success rate but it has an effect on the distribution of individual attack success rates.
The interquartile range narrows when 80\% of the attackers all escalate, but returns to equilibrium once all attackers escalate to 100\% to 0.55 (i.e. when there is no longer discrepancy or steep gradient in attacker strategies): this is in-line with the expectation that individual attack success rates would be skewed to be higher towards backdoor trigger patterns of higher relative frequency against other triggers due to imbalance of loss terms (Eqt \ref{equation:4}).
% that once there is no discrepancy or steep gradient where most attackers have $p=0.55$ while only a few still have $p=0.15$, then the playing field for trigger pattern saliency is balanced once more.
We also observe a cyclical pattern in the max accuracy w.r.t.  poisoned labels and outliers (black scatter points above the boxplot), where it tends to decrease when most attackers have escalated, but increase when few attackers relatively escalated, then return to an equilibrium level when either no attackers or all attacekers have escalated.
Escalation is an intriguing aspect of this attack, as the attack success rate has as much to do with the order in which attackers coordinate (whether cooperatively or selfishly), as it does with the backdoor trigger pattern.

\mybox{(E4)}
% \noindent\textbf{(Observation 7: Futility of backdoor trigger pattern \& target poison label coordination)}
% Gradual conformity in trigger selection (non-cooperative, cooperative)
In Table \ref{tab:coop1}, one of the variations we study is varying the overlap in target poison label selection between attackers.
Trigger patterns are randomly generated, and the distance between them is strongly correlated with the perturbation rate $\varepsilon$.
% , so we factor in this variance to show that this pattern is consistent and robust.
Regardless of $\varepsilon$, trigger distance w.r.t. shape and/or colour, or number of attackers; we find that if all $N$ attackers share the same trigger label, then a multi-agent backdoor attack can be successful (high collective accuracy w.r.t. poisoned labels).
There is a stark discrepancy in the range of values between each attacker picking different labels against all attackers picking the same label. 
Our initial hypothesis would have attributed this to feature collision, however even when trigger patterns were distant from each other ($\varepsilon$=0.15, low feature collision), there is still a clear accuracy difference between identical and non-identical target poison labels. 
We further investigate this feature collision hypothesis in Table \ref{tab:coop2} and Figure \ref{fig:escalation} (left).
What is more, the retainment of this high attack success rate is mutually beneficial (i.e. maximized collective ASR).
From an undefended multi-agent backdoor attack perspective, this would be considered a successful attack. However, one critical component of the payoff functions is that the attacker strategies also must be robust against defender strategies.
Unfortunately for attackers, the worst-performing backdoor defense
% (according to Experiments \ref{3.5}) 
cuts the attack success rate by a large margin; the collective ASR may not be as low as other label overlap settings under this defense, but it still is significantly lower than \textit{No Defense} cases.
% {\color{blue} To further support this conjecture and why not to underestimate the importance of defender strategies in determining success of an attack, 
% the definition and computation of the Nash equilibrium dictates that an agent's strategy is the equilibrium if the strategy payoff value cannot be further increased given the entire range of opponent strategies. 
% In this case, the dominant strategy of the defender is to enforce a backdoor defense, and no attack configuration is demonstrated where the mean payoff of this strategy would be lower than to not enforce a defense: this means we need to evaluate configurations with respect to a defender picking this strategy, and the equilibrium case where attacker(s) can maximize their payoff(s) is if they coordinate their trigger label selection, resulting in a mean (attackers, defender) equilibrium payoff of (25.4, 74.6)\%.
% }
Hence, we would argue that coordinating constant labels amongst attackers is not a robust strategy.

% In addition, we show the converse, that escalation 
In addition, we show that non-cooperatively/selfishly 
escalating $\varepsilon$ and/or
choosing 
target poison labels
% trigger patterns 
to be non-identical and personalized to each attacker's respective private datasets acts against individual and collective ASR. In practical settings, not only will private datasets encounter sub-population shift or domain shift, they may also have heteregeneous class/sub-class sets (i.e. attackers may wish to poison labels that are very specific to them, but not contained in other attacker's sets). 
For example, in a dataset containing a class 'dogs', there may be numerous sub-classes of dogs; so even though a set of attackers share the same class set, if they share different sub-class sets and each attempt to poison a target label that is contained in other attacker private datasets but is not selected for poisoning, then they are hindering themselves as well as other attacker ASRs.
It has been indicated thus far that the target poison label selection has a greater impact than the backdoor trigger pattern generation, so even if an attacker poisons a very niche sub-class, if the poisoned input is assigned a common/shared class, which may be the case if it is human-labeled by defender, then the backfiring effect will still manifest. 

% While on the topic of trigger pattern overlap, 
Some of the aforementioned patterns do not manifest when trigger patterns are orthogonal to each other (Table \ref{tab:coop2}).
Regardless of $\varepsilon$ changes (e.g. $0.55 \rightarrow 0.95$), orthogonally-coordinated trigger patterns do not sustain comparatively high ASR as that generated randomly, regardless of target poison label overlap.
% {\color{blue} What is puzzling is that the cosine distance is comparatively high as that when the poison rate is low. 
% What could cause this? Is it something to do with orthonormal and centroid distances?
% If we refer to the insight on orthogonal gradient descent (https://arxiv.org/pdf/2106.15023.pdf), they show that the interference between 2 distant inputs can be resolved by computing orthogonal losses. This would be in-line with both the super-position paper and our results w.r.t. clean labels accuracy, if we can show that orthogonal triggers (w.r.t. Eqt3 on loss) results in orthogonal loss components that inadvertently results in orthogonal gradient descent.
% }
Our hypothesis is that the target label overlap has a significant beneficial effect on collective ASR only when the trigger patterns are close to each other in the feature space (i.e. when cosine distance is low). 
% This is the consistent pattern thus far.
In general, we observe that the collective attack success rate is inversely proportional to the cosine distance of backdoor trigger patterns between attackers.

In addition, we wished to observe whether there is any benefit to attackers cooperating in sub-groups to coordinate trigger label selection. In both Tables, we find that when 40\% of attackers choose the same target label, there is no clear unilateral increase in their individual ASR compared to the other attackers; in fact, some other non-cooperating attackers may even have higher individual ASR. 
Though a gradual shift towards overlapping target poison labels did not yield a clear pattern when $N=5$, in the $N=100$ case there is a clearer proportionality where when the number of attackers is very large, when the sub-group of attackers coordinating their target labels increase, the collective ASR tends to increase.
We also attribute this phenomenon in $N=5$ to the notion that the proportion of trigger label overlap had not reached a critical threshold, and non-cooperating attackers happened to have trigger patterns more salient for their target label than even cooperating ones.
We demonstrate this threshold effect in Figure \ref{fig:escalation} (left), where if the proportion of attackers coordinating their labels is less than 80\%, then the distribution of individual ASRs are extremely wide; there is some indication that some attackers may be able to enjoy high ASR given the consistently increasing max and upper-quartile values as the proportion of overlapping participants increase, but as shown in Table \ref{tab:coop1} this does not guarantee that the participating colluders will necessarily reap this benefit.
Hence it generalizes a pattern of equity: the only times the collective ASR drops is when there is gross inequity between attackers (where some attackers have not escalated yet); when all attackers escalate again, the distribution of ASR resumes back to equilibrium.



% \item Coordination of trigger pattern distance, both shape (very important, clash on same pixel positions) and colour (anti-cooperative, cooperative)
% Now we would like to 
We consider cooperation with respect to trigger pattern generation. Though the random trigger pattern adaptation of BadNet renders unique patterns, it is clear from Table \ref{tab:coop1} that the resulting distance between the patterns varies on many factors such as perturbation rate. 
% Based on the notion of interference minimization (as the loss function we discussed in section \ref{} aligns with the transfer-interference tradeoff cited in \cite{})
Based on minimizing loss interference (Eqt \ref{equation:7}), we would like each attacker to generate trigger patterns that do not interfere with each other (i.e. orthogonal to each other, and reside in distinctly separate and distance subspaces from each other in the input space) regardless of factors such as perturbation rate. 
This is enabled from information sharing.
% As mentioned before, we do not conclude this to be a cooperative attack based on an assumption that the attack will be successful (so do not hold it against the results that they are invalid simply because the attack failed), we presume it as such because of information sharing, motivated by equations \ref{}.
The results indicate that information sharing with respect to trigger pattern orthogonality still does not yield favourable collective ASR. 
We verify that the shape distance is large (i.e. the positional indices of each perturbed pixel is also distinctly distant) as well as the colour+shape distance.
However, in all such cases, the collective ASR stays low, even when there is 100\% trigger label overlap. 
Consequently, this supports the empirical evidence and theoretical reasoning thus far that the true issue is not a feature collision between trigger patterns, else this attack would have been successful.
While this is just one of a few information sharing strategies evaluated (the other being on target trigger label), these results do not conclude that there does not exist an information sharing strategy that can unilaterally cause a successful multi-agent backdoor attack; instead, we introduce information sharing variants to evaluate the introduction of the attack, as well as the feature collision hypothesis.

\input{tables/cooperation}

% The final (but not tabulated separately) 
Another form of information sharing resulting in a cooperative attack is one where attackers coordinate such that they all share 1 identical backdoor trigger pattern and 1 identical target poison label, i.e. they collectively approximate a single-agent attack. The ASR is approximately that of a single-agent backdoor attack. Other than the downside of not being able to flexibly curate the attack to their needs (e.g. targeted misclassification), single-agent backdoor attacks have been shown in literature as well as \mybox{(E5)} to be mitigatable, hence this 
% extreme extent of 
information sharing strategy also does not yield a successful attack.
In fact, an extension of this is shown in Table \ref{tab:coop1}, where we have a set of low-distance trigger patterns, inadvertently due to a high $\varepsilon$.
It shows that if a set of attackers were to coordinate such they minimized the cosine distance between their backdoor trigger patterns, (i) if each attacker were to pick distinctly different target poison labels, the successful individual ASR would be random (as indicated where 1 attacker had a successful ASR while the others reached ASR=0.0), and (ii) if all attackers picked the same target poison label, then even though the backdoor trigger pattern is not identical, the ASR for these agents would still be collectively high.
This is in-line with results from \cite{9211729}, where the authors 
implemented 2 single-agent backdoor attacks with multiple trigger patterns with expectedly low distance from each other (one attack where the trigger patterns are of varying intensity of one pattern; another attack where they compose different sub-patterns, and thus different combinations of these sub-patterns would compose different triggers of low-distance to each other), and demonstrated that the attack success rate can be retained to be high, in addition to being more resilient against backdoor defenses.
Intuitively, our result for low-distance trigger patterns with same shared labels make sense, as there is no collision in features. The trigger pattern features overlap means there is a trigger sub-region (or overlapping region between trigger patterns) that becomes even \textit{more} salient and is reinforced during training (a robust backdoor trigger pattern/sub-pattern).
One could have argued that an optimal multi-agent backdoor strategy would be minimize cosine distance, where if attackers generate patterns of low orthogonality, then the trigger label cooperation case can maximize their collective ASR.
However, a cooperative attack with non-orthogonal triggers but same label can reduce their ASR to 0 with the inclusion of a backdoor defense due to it approximating a single-agent backdoor attack, regardless of a robust trigger sub-region. This cooperative setting may even be the weakest setting, weak because it requires attackers to share information that can be used against them (e.g. anti-cooperative behaviour such as escalation), and weak because of how easily it can be defended against.
% * Warning: At HIGH poison rates, the similarity of trigger patterns is extremely high due to large size of the trigger pattern	



% \noindent\textbf{(Observation 3: Resilient adversarial perturbations)}
% % \noindent\textbf{(Observation 5: Unaffected adversarial attack, if no trigger)}
% \mybox{(E3: \{adversarial, stylized\})}
% % Considering a poisoned dataset but a lack of backdoor trigger during run-time (i.e. run-time poison rate 0.0), we acknowledge that with the clean-label accuracy is stable for both stylization $\alpha$ attributed to the early-stopping training scheme. 
% For run-time poison rate 0.0,
% after adversarial attack (where both adversarial and stylized perturbations exist), we observe no significant difference as $\alpha$ varies.
% % between the tables between $\alpha=0.0$ and $\alpha=1.0$. 
% This indicates that the generation of adversarial perturbations with respect to a private dataset, even one with texture shift from other private datasets, can still retain a high adversarial attack success rate (low accuracy w.r.t. clean labels) in a multi-agent backdoor attack. 
% Additionally this gives the insight that an attacker can still pursue an adversarial attack strategy despite multiple agents; however, this may not necessarily always be practical, as the adversarial attack may not return a targeted misclassification of a specific target label (as evaluated in this experiment). 


% % \noindent\textbf{(Observation 4: Interference between backdoor and adversarial perturbations)}
% % Second, we evaluate the shift combination of \{backdoor, adversarial\}.
% \mybox{(E3: \{backdoor, adversarial\})}
% At $N=1$, 
% % we also note some interesting patterns in 
% we observe how adversarial perturbations sometimes contribute or hinder a backdoor attack in terms of accuracy w.r.t. poisoned labels: 
% specifically studying the range $\varepsilon_{\textnormal{b}}, p: 0.2, 0.4, 0.8$ across $\varepsilon_{\textnormal{a}}: 0.2, 0.4, 0.8, 1.0$, we find that at low $\varepsilon_{\textnormal{b}}, p$ an increasing $\varepsilon_{\textnormal{a}}$ contributes to and increases the backdoor ASR, but at high $\varepsilon_{\textnormal{b}}, p$ an increasing $\varepsilon_{\textnormal{a}}$ hinders and decreases the backdoor ASR.
% There appears to be some form of interference taking place between the adversarial perturbations and backdoor perturbations: our hypothesis on this phenomenon is that when the poison rate is low against the surrogate model's gradients, FGSM is optimized towards pushing the inputs \textit{towards} the poisoned label, but when the poison rate is high then FGSM is optimized towards pushing inputs \textit{away} from the poisoned label. 
% This appears to be counter-intuitive; from FGSM's point-of-view, the backdoor trigger presence should return perturbations that push the input's classification as far away from the poison label as possible (since from FGSM's viewpoint, the poison label is the ground-truth that it is trying to misclassify; however, FGSM does not take the ground-truth label as an argument, but instead infers it from the gradients).


% % \noindent\textbf{(Observation 4 cont'd)}
% % Finally, we evaluate the shift combination of \{backdoor, adversarial, stylized\}.
% \mybox{(E3: \{backdoor, adversarial, stylized\})}
% For low backdoor $\varepsilon_{\textnormal{b}}, p$, the adversarial $\varepsilon_{\textnormal{a}}$ contributes to increasing the accuracy w.r.t. poisoned labels, i.e. improving the backdoor ASR. This is consistent across stylization and number of attackers, except for $N=100, \alpha=1.0$.
% However for higher values of $\varepsilon_{\textnormal{b}}, p$ at $N=1$, we note that after a threshold of $\varepsilon_{\textnormal{a}} \geq 0.4$, adversarial perturbations counter the backdoor attack for $\alpha=0.0$. For $\alpha=1.0, N=1$, $\varepsilon_{\textnormal{a}}$ continues to incrementally improve the backdoor attack.
% For $N=100$, regardless of stylization, at high $\varepsilon_{\textnormal{b}}, p$, changes in $\varepsilon_{\textnormal{a}}$ do not significantly change the accuracy w.r.t. poisoned labels.
% % All of the 3 aforementioned patterns are identical and consistent with the patterns in \{backdoor, stylized\}, hence it leads us to believe that these changes are driven by stylistic perturbations rather than adversarial perturbations. 


% \noindent\textbf{(Observation 4: Increasingly-distant model parameters)}
% % \noindent\textbf{Findings. }
% \mybox{(E6)}
% The values of the biases for most layers have not changed significantly and fall under the distance region $0.0 - 0.1$. 
% For the first convolutional layer ($\texttt{Conv2d0}$) weights, 
% we observe that the weights change significantly as soon as an additional attacker is introduced: the weights for $N=10, 100, 1000$ are closer to each other, and only $N=1$ has a distinctly large distance from all others.
% It implies that the backfiring effect is immediate
% % , and the tradeoff between ASR and number of attackers occurs 
% as soon as $N>1$. 
% In addition, it does not indicate a significant diminishing marginal effect, where the weights distance change is significant with respect to an increase in attackers. 

% The pattern for $\texttt{Conv2d0}$ is exacerbated in $\texttt{Conv2d1}$ and $\texttt{Conv2d2}$.
% There is a very clear trend, where although the distance reduction is not as linear in $\texttt{Conv2d0}$, it is clearly linear the further we go down the layers in the network, where: for the weights of a layer for 2 different models trained under 2 distinct attacker configurations (different $N_0$, $N_1$), the further that $N_0$ and $N_1$ are jointly distant from 1, the closer their cosine distance is. The further down the convolutional layer indices we evaluate, the distance differentials become more stark and distinct. 

% We observe that the distance patterns for the cosine distance with respect to the full network parameters, mask of the lottery ticket, and parameters of the lottery ticket are all extremely similar: this implies to us that the main driving changes to the optima computed (and the main driver for the distance between weights in the full network) is specifically attributed to the changes in the lottery ticket required to resolve the backdoor trigger pattern. It follows through on our previous analysis, that the main driving factor for the DNN optimization is the insertion or rejection of a subnetwork.

% For all the fully-convolution layers (weights as well as biases), we observe a pattern where the lottery ticket drives the distance outcomes across all 3 cosine distance matrices.
% We also observe an asymmetrical pattern compared to the convolutional layers, where the further down the fully-connected layer indices we evaluate, the distance differentials become less stark. In earlier $\texttt{fc}$ layers, there is a similar pattern to the $\texttt{Conv2d}$ layers, where the further that $N_0$ and $N_1$ are jointly distant from 1, the closer their cosine distance is. 


==> tables/figures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Table 5	Vary by dataset
\begin{table*}

\parbox{.5\linewidth}{
\centering

% \resizebox{0.5\textwidth}{0.06\textheight}{
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{|lcccc|}
\hline
& \multicolumn{4}{c|}{
\textit{$N=1$}
} 
\\ \hline
Dataset 
& \textit{MNIST}            
& \textit{SVNH}            
& \textit{CIFAR10}           
& \textit{STL10}            
\\ \hline

\multicolumn{1}{|p{3cm}|}{Defender Validation Acc (Post-Backdoor)}   
& {\color{black} $99.7$}
& {\color{black} $92.1$}
& {\color{black} $84.5$}
& {\color{black} $95.4$}
\\ \hline

\multicolumn{1}{|p{3cm}|}{Run-time Acc w.r.t. poisoned labels}   
& {\color{black} $100.0$}
& {\color{black} $98.1$}
& {\color{black} $89.8$}
& {\color{black} $100.0$}
\\ \hline

\multicolumn{1}{|p{3cm}|}{Run-time Acc w.r.t. clean labels}   
& {\color{black} $10.4$}
& {\color{black} $9.9$}
& {\color{black} $13.0$}
& {\color{black} $10.9$}
\\ \hline

\end{tabular}
}

\caption{Foo}
}
\hfill
\parbox{.5\linewidth}{
\centering

% \resizebox{0.5\textwidth}{2.5em}{
% \resizebox{0.5\textwidth}{0.06\textheight}{
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|lcccc|}
\hline
& \multicolumn{4}{c|}{
\textit{$N=100$}
} 
\\ \hline
Dataset 
& \textit{MNIST}            
& \textit{SVNH}            
& \textit{CIFAR10}           
& \textit{STL10}            
\\ \hline

\multicolumn{1}{|p{3cm}|}{Defender Validation Acc (Post-Backdoor)}   
& {\color{black} $99.7$}
& {\color{black} $91.9$}
& {\color{black} $84.6$}
& {\color{black} $71.9$}
\\ \hline

\multicolumn{1}{|p{3cm}|}{Run-time Acc w.r.t. poisoned labels}   
& {\color{black} $100.0 \pm 0.0$}
& {\color{black} $12.3 \pm 19.1$}
& {\color{black} $12.1 \pm 14.0$}
& {\color{black} $12.6 \pm 15.4$}
\\ \hline

\multicolumn{1}{|p{3cm}|}{Run-time Acc w.r.t. clean labels}   
& {\color{black} $9.6 \pm 3.0$}
& {\color{black} $10.4 \pm 3.2$}
& {\color{black} $15.5 \pm 4.6$}
& {\color{black} $10.0 \pm 10.2$}
\\ \hline

\end{tabular}
}

\caption{Bar}
}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Capacity
\begin{table*}
	\begin{minipage}{0.32\textwidth}
		\centering
		\resizebox{\textwidth}{!}{
        \begin{tabular}{|lcc|}
        \hline
        Name 
        & \textit{Number of parameters}            
        & \textit{Ratio w.r.t ResNet18}               
        \\ \hline
        
         \tikz\draw[smallcnn,fill=smallcnn] (0,0) circle (.5ex); SmallCNN
        & {\color{black} 15,722}
        & {\color{black} 0.0014}
        \\ \hline
        
         \tikz\draw[resnet9,fill=resnet9] (0,0) circle (.5ex); ResNet9
        & {\color{black} 7,756,554}
        & {\color{black} 0.6936}
        \\ \hline
        
         \tikz\draw[resnet18,fill=resnet18] (0,0) circle (.5ex); ResNet18
        & {\color{black} 11,181,642}
        & {\color{black} 1.0000}
        \\ \hline
        
         \tikz\draw[resnet34,fill=resnet34] (0,0) circle (.5ex); ResNet34
        & {\color{black} 21,289,802}
        & {\color{black} 1.9040}
        \\ \hline
        
         \tikz\draw[resnet50,fill=resnet50] (0,0) circle (.5ex); ResNet50
        & {\color{black} 23,528,522}
        & {\color{black} 2.1042}
        \\ \hline
        
         \tikz\draw[resnet101,fill=resnet101] (0,0) circle (.5ex); ResNet101
        & {\color{black} 42,520,650}
        & {\color{black} 3.8027}
        \\ \hline
        
         \tikz\draw[resnet152,fill=resnet152] (0,0) circle (.5ex); ResNet152
        & {\color{black} 58,164,298}
        & {\color{black} 5.2018}
        \\ \hline
        
         \tikz\draw[wide_resnet50_2,fill=wide_resnet50_2] (0,0) circle (.5ex); W-ResNet50
        & {\color{black} 66,854,730}
        & {\color{black} 5.9790}
        \\ \hline
        
         \tikz\draw[wide_resnet101_2,fill=wide_resnet101_2] (0,0) circle (.5ex); W-ResNet101
        & {\color{black} 124,858,186}
        & {\color{black} 11.1664}
        \\ \hline
        
         \tikz\draw[vgg,fill=vgg] (0,0) circle (.5ex); VGG
        & {\color{black} 128,812,810}
        & {\color{black} 11.5200}
        \\ \hline
        
        \end{tabular}
        }
	\end{minipage}\hfill
	\begin{minipage}{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{assets/capacity_1.pdf}
	\end{minipage}
	\begin{minipage}{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{assets/capacity_2.pdf}
	\end{minipage}
	\caption{A table beside a figure}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Defenses

% \begin{minipage}{0.4\textwidth}
% \centering
% \includegraphics[width=\textwidth]{assets/defenses_n1.pdf}
% \end{minipage}
% \begin{minipage}{0.4\textwidth}
% \centering
% \includegraphics[width=\textwidth]{assets/defenses_n100.pdf}
% \end{minipage}

\begin{figure}[]
    \centering
    \includegraphics[width=0.5\textwidth]{assets/defenses_n1.pdf}
    \includegraphics[width=0.5\textwidth]{assets/defenses_n100.pdf}
    \caption{}
    \label{fig:archi}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Adv vs Backdoor vs Stylistic

% \begin{minipage}{0.4\textwidth}
% \centering
% \includegraphics[width=\textwidth]{assets/defenses_n1.pdf}
% \end{minipage}
% \begin{minipage}{0.4\textwidth}
% \centering
% \includegraphics[width=\textwidth]{assets/defenses_n100.pdf}
% \end{minipage}

\begin{figure*}[]
    \centering
    \includegraphics[width=0.245\textwidth]{assets/n1_a0_before.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n1_a0_after.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n100_a0_before.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n100_a0_after.pdf}
    
    
    
    \includegraphics[width=0.245\textwidth]{assets/n1_a5_before.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n1_a5_after.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n100_a5_before.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n100_a5_after.pdf}
    
    \includegraphics[width=0.245\textwidth]{assets/n1_a10_before.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n1_a10_after.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n100_a10_before.pdf}
    \includegraphics[width=0.245\textwidth]{assets/n100_a10_after.pdf}

    \caption{}
    \label{fig:archi}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% poison rate vs epsilon (vs num attackers)

\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{assets/heatmap.pdf}
    \caption{}
    \label{fig:archi}
\end{figure*}

% \begin{tikzpicture}[scale=0.6]

% %   \node at (5,0) {$N = 10^0$};
% %   \node at (5,0) {Backdoor epsilon};
%   \foreach \y [count=\n] in {
%       {74,25,39,20,3,3,3,3,3},
%       {25,53,31,17,7,7,2,3,2},
%       {39,31,37,24,3,3,3,3,3},
%       {20,17,24,37,2,2,6,5,5},
%       {3,7,3,2,12,1,0,0,0},
%       {3,7,3,2,1,36,0,0,0},
%       {3,2,3,6,0,0,45,1,1},
%       {3,3,3,5,0,0,1,23,1},
%       {3,2,3,5,0,0,1,1,78},
%     } {
%       \foreach \x [count=\m] in \y {
%         \node[fill=good_ASR!\x!bad_ASR, minimum size=6mm, text=white] at (\m,-\n) {\x};
%       }
%     }
% \end{tikzpicture}


% \begin{table*}

% % \resizebox{0.5\textwidth}{0.06\textheight}{
% \resizebox{0.4\textwidth}{!}{
% {\renewcommand{\arraystretch}{2.3}
% \begin{tabular}{|ccccccc|}
% \hline
% \multicolumn{7}{|c|}{
% \textit{$N=10^0$}
% } 
% \\ \hline
% & \multicolumn{6}{c|}{
% Backdoor epsilon
% } 
% \\ 
% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Poison rate}}}
% &
% & $0.1$
% & $0.2$
% & $0.4$
% & $0.8$
% & $1.0$
% \\ 

% & $0.1$
% & 
% \multicolumn{5}{c}{\multirow{5}{*}{
% \begin{tikzpicture}[scale=0.95]

%   \foreach \y [count=\n] in {
%       {11.5,22.5,65.4,94.0,100},
%       {19.8,40.4,80.1,92.8,100},
%       {24.3,44.6,78.7,93.6,100},
%       {24.5,42.1,85.8,95.3,100},
%       {36.4,58.4,88.6,95.0,100},
%     } {
%       \foreach \x [count=\m] in \y {
%         \node[fill=bad_ASR!\x!good_ASR, minimum size=10mm, text=white] at (\m,-\n) {\x};
%       }
%     }
% \end{tikzpicture}
% }}
% \\ 

% & $0.2$
% \\

% & $0.4$
% \\ 

% & $0.8$
% \\

% & $1.0$
% \\ \hline

% \end{tabular}
% }
% }
% % \caption{Bar}

% \end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Cooperation / "Orthogonality"
% const trigger vs distinct triggers

\begin{table*}
\tiny
\centering
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|l|ccccc|}
\multicolumn{1}{c}{}   
\\ \hline
Agent 
\\ \hline

Trigger shape cosine distance w.r.t. Agent 1
\\ \hline

Trigger (shape + colour) cosine distance w.r.t. Agent 1
\\ \hline

Trigger label
\\ \hline

Backdoor epsilon
\\ \hline

Real poison rate (during training)
\\ \hline

Run-time Acc w.r.t. poisoned labels
\\ \hline

Run-time Acc w.r.t. clean labels
\\ \hline

Trigger label
\\ \hline

Backdoor epsilon
\\ \hline

Real poison rate (during training)
\\ \hline

Run-time Acc w.r.t. poisoned labels
\\ \hline

Run-time Acc w.r.t. clean labels
\\ \hline

Trigger label
\\ \hline

Backdoor epsilon
\\ \hline

Real poison rate (during training)
\\ \hline

Run-time Acc w.r.t. poisoned labels
\\ \hline

Run-time Acc w.r.t. clean labels
\\ \hline


\end{tabular}
}

% \caption{fig}
}
% \hfill
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|ccccc|}

\hline
\multicolumn{5}{|c|}{No defense, N=5, p=0.032, eps=0.15}   
\\ \hline
\textit{1}            
& \textit{2}            
& \textit{3}           
& \textit{4}
& \textit{5}
\\ \hline

$0.0$
& $0.849$
& $0.849$
& $0.873$
& $0.785$
\\ \hline

$0.0$
& $0.904$
& $0.883$
& $0.895$
& $0.819$
\\ \hline

$0$
& $2$
& $4$
& $6$
& $8$
\\ \hline

$0.15$
& $0.15$
& $0.15$
& $0.15$
& $0.15$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$3.9$
& $14.4$
& $9.7$
& $36.3$
& $8.7$
\\ \hline

$23.9$
& $29.7$
& $27.6$
& $28.4$
& $24.9$
\\ \hline

$2$
& {\color{red}$4$}
& {\color{red}$4$}
& $6$
& $8$
\\ \hline

$0.15$
& $0.15$
& $0.15$
& $0.15$
& $0.15$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$6.9$
& $18.9$
& $21.2$
& $30.4$
& $9.9$
\\ \hline

$25.1$
& $28.8$
& $28.1$
& $27.2$
& $24.9$
\\ \hline

{\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
\\ \hline

$0.15$
& $0.15$
& $0.15$
& $0.15$
& $0.15$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$38.3$
& $33.4$
& $38.8$
& $29.9$
& $50.4$
\\ \hline

$24.8$
& $27.1$
& $26.5$
& $26.4$
& $21.9$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}
% \hfill
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|ccccc|}

\hline
\multicolumn{5}{|c|}{No defense, N=5, p=0.032, eps=0.55}   
\\ \hline
\textit{1}            
& \textit{2}            
& \textit{3}           
& \textit{4}
& \textit{5}
\\ \hline


$0.0$
& $0.458$
& $0.454$
& $0.456$
& $0.445$
\\ \hline

$0.0$
& $0.598$
& $0.572$
& $0.580$
& $0.582$
\\ \hline

$0$
& $2$
& $4$
& $6$
& $8$
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$3.4$
& $14.6$
& $3.4$
& $9.9$
& $1.8$
\\ \hline

$15.2$
& $11.9$
& $13.3$
& $14.1$
& $12.4$
\\ \hline

$2$
& {\color{red}$4$}
& {\color{red}$4$}
& $6$
& $8$
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$62.2$
& $16.4$
& $8.3$
& $10.8$
& $4.8$
\\ \hline

$12.9$
& $16.2$
& $10.9$
& $13.2$
& $13.3$
\\ \hline

{\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$89.3$
& $97.6$
& $89.3$
& $96.1$
& $96.1$
\\ \hline

$11.1$
& $11.2$
& $10.8$
& $9.7$
& $10.2$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}
% \hfill
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|ccccc|}

\hline
\multicolumn{5}{|c|}{No defense, N=5, p=0.032, eps=0.95}   
\\ \hline
\textit{1}            
& \textit{2}            
& \textit{3}           
& \textit{4}
& \textit{5}
\\ \hline


$0.0$
& $0.053$
& $0.046$
& $0.044$
& $0.049$
\\ \hline

$0.0$
& $0.286$
& $0.283$
& $0.282$
& $0.283$
\\ \hline

$0$
& $2$
& $4$
& $6$
& $8$
\\ \hline

$0.95$
& $0.95$
& $0.95$
& $0.95$
& $0.95$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$75.9$
& $18.6$
& $0.2$
& $61.7$
& $0.0$
\\ \hline

$7.8$
& $10.3$
& $11.6$
& $8.9$
& $11.3$
\\ \hline

$2$
& {\color{red}$4$}
& {\color{red}$4$}
& $6$
& $8$
\\ \hline

$0.95$
& $0.95$
& $0.95$
& $0.95$
& $0.95$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$2.7$
& $9.6$
& $81.2$
& $3.7$
& $0.0$
\\ \hline

$12.7$
& $10.4$
& $9.6$
& $9.3$
& $10.2$
\\ \hline

{\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
\\ \hline

$0.95$
& $0.95$
& $0.95$
& $0.95$
& $0.95$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$100.0$
& $91.8$
& $100.0$
& $100.0$
& $100.0$
\\ \hline

$10.4$
& $12.2$
& $9.4$
& $9.4$
& $10.1$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}
% \hfill
\parbox{.0715\linewidth}{
\centering

\resizebox{0.0715\textwidth}{!}{

\begin{tabular}{|c|}

\hline
\multicolumn{1}{|c|}{N=100 (Avg)}   
\\ \hline
\textit{1...100}            
\\ \hline

$0.453$
\\ \hline

$0.583$
\\ \hline

$20\{0,2,4,6,8\}$
\\ \hline

$0.55$
\\ \hline

$0.032$
\\ \hline

$20.4 \pm 15.8$
\\ \hline

$12.3 \pm 3.92$
\\ \hline

${\color{red}40\{4\}}, 20\{2, 6, 8\}$
\\ \hline

$0.55$
\\ \hline

$0.032$
\\ \hline

$30.8 \pm 24.8$
\\ \hline

$11.1 \pm 3.29$
\\ \hline

${\color{red}100\{4\}}$
\\ \hline

$0.55$
\\ \hline

$0.032$
\\ \hline

$19.9 \pm 14.6$
\\ \hline

$12.4, 3.58$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}
% \hfill
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|ccccc|}

\hline
\multicolumn{5}{|c|}{Defense method: Backdoor Adversarial training}   
\\ \hline
\textit{1}            
& \textit{2}            
& \textit{3}           
& \textit{4}
& \textit{5}
\\ \hline


$0.0$
& $0.458$
& $0.454$
& $0.456$
& $0.445$
\\ \hline

$0.0$
& $0.598$
& $0.572$
& $0.580$
& $0.582$
\\ \hline

$0$
& $2$
& $4$
& $6$
& $8$
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$9.8$
& $9.6$
& $4.4$
& $47.5$
& $5.6$
\\ \hline

$13.6$
& $13.3$
& $14.2$
& $14.6$
& $15.1$
\\ \hline

$2$
& {\color{red}$4$}
& {\color{red}$4$}
& $6$
& $8$
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$7.2$
& $23.0$
& $14.7$
& $38.4$
& $7.0$
\\ \hline

$11.1$
& $14.4$
& $15.79$
& $14.2$
& $14.2$
\\ \hline

{\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$26.7$
& $31.7$
& $12.9$
& $51.7$
& $13.9$
\\ \hline

$12.6$
& $12.9$
& $12.2$
& $14.1$
& $13.2$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}

\caption{Cooperation setting 1: Trigger patterns of low distance / No cooperation}
\end{table*}

\begin{table*}
\tiny
\centering
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|l|ccccc|}
\multicolumn{1}{c}{}   
\\ \hline
Agent 
\\ \hline

Trigger shape cosine distance w.r.t. Agent 1
\\ \hline

Trigger (shape + colour) cosine distance w.r.t. Agent 1
\\ \hline

Trigger label
\\ \hline

Backdoor epsilon
\\ \hline

Real poison rate (during training)
\\ \hline

Run-time Acc w.r.t. poisoned labels
\\ \hline

Run-time Acc w.r.t. clean labels
\\ \hline

Trigger label
\\ \hline

Backdoor epsilon
\\ \hline

Real poison rate (during training)
\\ \hline

Run-time Acc w.r.t. poisoned labels
\\ \hline

Run-time Acc w.r.t. clean labels
\\ \hline

Trigger label
\\ \hline

Backdoor epsilon
\\ \hline

Real poison rate (during training)
\\ \hline

Run-time Acc w.r.t. poisoned labels
\\ \hline

Run-time Acc w.r.t. clean labels
\\ \hline


\end{tabular}
}

% \caption{fig}
}
% \hfill
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|ccccc|}

\hline
\multicolumn{5}{|c|}{No defense, N=5, p=0.032, eps=0.15}   
\\ \hline
\textit{1}            
& \textit{2}            
& \textit{3}           
& \textit{4}
& \textit{5}
\\ \hline

$0.0$
& $1.0$
& $1.0$
& $1.0$
& $0.996$
\\ \hline

$0.0$
& $0.955$
& $1.0$
& $0.988$
& $0.974$
\\ \hline

$0$
& $2$
& $4$
& $6$
& $8$
\\ \hline

$0.15$
& $0.15$
& $0.15$
& $0.15$
& $0.15$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$9,6$
& $12.6$
& $11.0$
& $6.8$
& $11.1$
\\ \hline

$58.2$
& $56.4$
& $54.6$
& $57.8$
& $57.2$
\\ \hline

$2$
& {\color{red}$4$}
& {\color{red}$4$}
& $6$
& $8$
\\ \hline

$0.15$
& $0.15$
& $0.15$
& $0.15$
& $0.15$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$10.1$
& $11.9$
& $10.8$
& $9.9$
& $9.8$
\\ \hline

$58.5$
& $58.1$
& $56.6$
& $57.8$
& $57.2$
\\ \hline

{\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
\\ \hline

$0.15$
& $0.15$
& $0.15$
& $0.15$
& $0.15$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$12.1$
& $11.7$
& $10.7$
& $10.1$
& $11.7$
\\ \hline

$59.0$
& $56.7$
& $56.0$
& $57.1$
& $56.8$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}
% \hfill
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|ccccc|}

\hline
\multicolumn{5}{|c|}{No defense, N=5, p=0.032, eps=0.55}   
\\ \hline
\textit{1}            
& \textit{2}            
& \textit{3}           
& \textit{4}
& \textit{5}
\\ \hline


$0.0$
& $0.897$
& $1.0$
& $1.0$
& $0.959$
\\ \hline

$0.0$
& $1.0$
& $1.0$
& $0.994$
& $0.975$
\\ \hline

$0$
& $2$
& $4$
& $6$
& $8$
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$10.2$
& $11.5$
& $11.6$
& $8.8$
& $10.3$
\\ \hline

$60.0$
& $58.3$
& $57.6$
& $58.5$
& $56.3$
\\ \hline

$2$
& {\color{red}$4$}
& {\color{red}$4$}
& $6$
& $8$
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$9.7$
& $13.3$
& $11.2$
& $10.4$
& $11.9$
\\ \hline

$58.1$
& $57.3$
& $56.3$
& $58.2$
& $57.5$
\\ \hline

{\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$15.2$
& $14.8$
& $15.0$
& $14.2$
& $14.8$
\\ \hline

$58.61$
& $56.7$
& $54.7$
& $56.4$
& $57.4$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}
% \hfill
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|ccccc|}

\hline
\multicolumn{5}{|c|}{No defense, N=5, p=0.032, eps=0.95}   
\\ \hline
\textit{1}            
& \textit{2}            
& \textit{3}           
& \textit{4}
& \textit{5}
\\ \hline


$0.0$
& $0.777$
& $1.0$
& $1.0$
& $0.918$
\\ \hline

$0.0$
& $1.0$
& $1.0$
& $0.971$
& $0.963$
\\ \hline

$0$
& $2$
& $4$
& $6$
& $8$
\\ \hline

$0.95$
& $0.95$
& $0.95$
& $0.95$
& $0.95$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$9.0$
& $10.3$
& $11.3$
& $8.4$
& $11.2$
\\ \hline

$57.7$
& $57.4$
& $56.4$
& $58.4$
& $57.1$
\\ \hline

$2$
& {\color{red}$4$}
& {\color{red}$4$}
& $6$
& $8$
\\ \hline

$0.95$
& $0.95$
& $0.95$
& $0.95$
& $0.95$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$7.7$
& $9.7$
& $9.6$
& $8.7$
& $13.8$
\\ \hline

$57.8$
& $58.5$
& $56.7$
& $58.1$
& $56.5$
\\ \hline

{\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
\\ \hline

$0.95$
& $0.95$
& $0.95$
& $0.95$
& $0.95$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$13.3$
& $13.4$
& $12.1$
& $11.3$
& $11.9$
\\ \hline

$57.9$
& $58.2$
& $56.1$
& $58.9$
& $57.8$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}
% \hfill
\parbox{.0715\linewidth}{
\centering

\resizebox{0.0715\textwidth}{!}{

\begin{tabular}{|c|}

\hline
\multicolumn{1}{|c|}{N=100 (Avg)}   
\\ \hline
\textit{1...100}            
\\ \hline

$1.0$
\\ \hline

$1.0$
\\ \hline

$20\{0,2,4,6,8\}$
\\ \hline

$0.55$
\\ \hline

$0.032$
\\ \hline

$10.0 \pm 3.58$
\\ \hline

$58.2 \pm 4.65$
\\ \hline

${\color{red}40\{4\}}, 20\{2, 6, 8\}$
\\ \hline

$0.55$
\\ \hline

$0.032$
\\ \hline

$9.96 \pm 2.96$
\\ \hline

$58.9 \pm 4.82$
\\ \hline

${\color{red}100\{4\}}$
\\ \hline

$0.55$
\\ \hline

$0.032$
\\ \hline

$9.41 \pm 3.11$
\\ \hline

$59.2, 5.79$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}
% \hfill
\parbox{.15\linewidth}{
\centering

\resizebox{0.15\textwidth}{!}{

\begin{tabular}{|ccccc|}

\hline
\multicolumn{5}{|c|}{Defense method: Backdoor Adversarial training}   
\\ \hline
\textit{1}            
& \textit{2}            
& \textit{3}           
& \textit{4}
& \textit{5}
\\ \hline


$0.0$
& $0.897$
& $1.0$
& $1.0$
& $0.959$
\\ \hline

$0.0$
& $1.0$
& $1.0$
& $0.994$
& $0.975$
\\ \hline

$0$
& $2$
& $4$
& $6$
& $8$
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$8.4$
& $9.2$
& $9.6$
& $7.4$
& $11.8$
\\ \hline

$50.8$
& $48.3$
& $49.4$
& $49.1$
& $49.1$
\\ \hline

$2$
& {\color{red}$4$}
& {\color{red}$4$}
& $6$
& $8$
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$9.2$
& $6.2$
& $7.1$
& $7.4$
& $11.6$
\\ \hline

$52.7$
& $49.9$
& $49.9$
& $49.6$
& $49.0$
\\ \hline

{\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
& {\color{red}$4$}
\\ \hline

$0.55$
& $0.55$
& $0.55$
& $0.55$
& $0.55$
\\ \hline

$0.032$
& $0.032$
& $0.032$
& $0.032$
& $0.032$
\\ \hline

$8.9$
& $8.7$
& $8.4$
& $9.5$
& $8.4$
\\ \hline

$51.0$
& $51.5$
& $49.7$
& $49.9$
& $49.9$
\\ \hline


\end{tabular}
}

% \caption{Bar}
}

\caption{Cooperation setting 2: Trigger patterns of high distance}
\end{table*}


